NVDiff: Graph Generation through the Diffusion of Node Vectors

Learning to generate graphs is challenging as a graph is a set of pairwise connected, unordered nodes encoding complex combinatorial structures. Recently, several works have proposed graph generative models based on normalizing flows or score-based diffusion models. However, these models need to generate nodes and edges in parallel from the same process, whose dimensionality is unnecessarily high. We propose NVDiff, which takes the VGAE structure and uses a score-based generative model (SGM) as a flexible prior to sample node vectors. By modeling only node vectors in the latent space, NVDiff significantly reduces the dimension of the diffusion process and thus improves sampling speed. Built on the NVDiff framework, we introduce an attention-based score network capable of capturing both local and global contexts of graphs. Experiments indicate that NVDiff significantly reduces computations and can model much larger graphs than competing methods. At the same time, it achieves superior or competitive performances over various datasets compared to previous methods.

==> NIPS/sections/abstract.tex <==


%   Learning to generate graph-structure data is challenging as graphs are discrete data with no intrinsic node orders  . Most of the previous works fail to capture the exchangeable property of the graph distribution. While several works successfully achieve this by proposing a permutation invariant model, they suffer either from the model expressivity or from the computational efficiency. To address those difficulties, we propose a score-based generative model (SGM) that models graphs in a latent space. \red{By utilizing SGM framework, we are able to have more freedom to choose model architecture thus improve the model expressivity. By mapping graph data to a latent space, we are able to train a SGM on a low-dimensional latent space, hence boost the sampling speed.} Specifically, we introduce multiple latent space encoding strategies, in the consideration of the model expressivity and model scalability. Then we introduce a attention-based score network that is designed for estimating scores for the graph generative problem. Experiments ..

\begin{abstract}

%Graph Generation through the Diffusion of Node Vectors

Learning to generate graphs is challenging as a graph is a set of pairwise connected, unordered nodes encoding complex combinatorial structures. Recently, several works have proposed graph generative models based on normalizing flows or score-based diffusion models. However, these models need to generate nodes and edges in parallel from the same process, whose dimensionality is unnecessarily high. We propose NVDiff, which takes the VGAE structure and uses a score-based generative model (SGM) as a flexible prior to sample node vectors. By modeling only node vectors in the latent space, NVDiff significantly reduces the dimension of the diffusion process and thus improves sampling speed. Built on the NVDiff framework, we introduce an attention-based score network capable of capturing both local and global contexts of graphs. Experiments indicate that NVDiff achieves superior or competitive performances over various datasets compared to previous methods. Moreover, our model significantly improves the sampling speed and can model larger graphs.

\end{abstract}


% \red{By mapping graph data to a latent space, we are able to obtain a more expressive generative model, inject graph domain knowledge into the model and train a SGM on a low-dimensional latent space, hence boost the sampling speed.}
% \begin{abstract}
%   Learning to generate graph-structure data is challenging as graphs are discrete data with no intrinsic node orders. Most of the previous works fail to capture the exchangeable property of the graph distribution. While several works successfully achieve this by proposing a permutation invariant model, they suffer either from the model expressivity or from the computational efficiency. To address those difficulties, we propose a score-based graph generative model that models graphs in a latent space. By mapping graph data to a latent space, we are able to obtain a more expressive generative model, bypass the problem of modeling the discrete data distribution with a continuous distribution, and train a SGM on a smoother low-dimensional latent space, hence stabilize the training procedure and boost the sampling speed. Specifically, we introduce multiple latent space encoding strategies, in the consideration of the model expressivity and model scalability. Then we introduce a attention-based score network that is designed for estimating scores for the graph generative problem. Experiments ..
% \end{abstract}

==> NIPS/sections/conclusions.tex <==
\vspace{-1em}
\section{Conclusions and limitations} \label{sec:conclude}
This paper introduces NVDiff that generates novel, realistic, and unique graphs by taking the VGAE structure and uses SGM as its prior for latent node vectors. NVDiff guarantees exchangeability without losing expressiveness by implementing SGM using attention-based networks. When pairing with a properly designed GNN decoder, SGM can sample complex graphs in one shot and enjoys a fast sampling speed.

This paper has the following limitations: (1) We setup NVDiff under the variational auto-encoder framework. VAE optimizes the lower bound of the likelihood function, which corresponds to the KL divergence between the empirical distribution and the parameterized distribution. Optimization under other objectives is not discussed. (2) Current NVDiff does not support conditional graph generation, which can be used for optimizing molecular property.


==> NIPS/sections/experiments.tex <==
\vspace{-1em}
\section{Experiments} \label{sec:exp}
% v1
% {In this section, we design a set of experiments to check whether the proposed method can generate high-quality graphs by using node vectors only. We also diagnose how node vectors are generated from the diffusion prior.}
% We demonstrate quantitative and qualitative results showing that NVDiff generates high-quality graphs with latent node vectors.
% \scriptupdate{In Section \ref{sec:exp-setup} we introduce the datasets, baselines and evaluation metrics used in the experiment. In Section \ref{sec:exp-quan}, we evaluate the quality of samples generated by different model as well as the sampling speed quantitatively. }
\scriptupdate{We design a set of experiments to demonstrate that NVDiff can generate high-quality graphs with latent node vectors. Specifically, in Section \ref{sec:exp-quan} we quantitatively evaluate the sample quality and sampling speed for selected baseline models and NVDiff over various metrics. In Section \ref{sec:exp-qual} we investigate NVDiff from the perspective of the generation dynamics, effectiveness of the contextual embedding, and graph visualization. More experiment results can be found in the Appendix \ref{app:extra-exp}.}
\vspace{-1em}
\subsection{Experiment Setup}
\label{sec:exp-setup}
Here we briefly discuss the datasets, baselines, and evaluation metrics we use in the experiments. Further details can be found in Appendix. \ref{app:exp-detail}.

\textbf{Datasets.} We use six datasets, including two molecular datasets and four generic graph datasets. For molecular datasets, we consider QM9 ~\citep{ramakrishnan2014quantum} and {ZINC250K} ~\citep{irwin2012zinc}. For generic graph datasets, we consider {Community} and {Ego} and the small versions of them. Detailed statistics about all datasets are provided in Appendix \ref{app:data-stats}.

%(statistics in appendix) We train and evaluate our model on two molecule datasets and four generic datasets. The two molecule datasets are QM9[] and Zinc250K[]. Zinc250k contains 250,000 molecules, which contain up to 38 atoms of 9 types. QM9 contains 133,885 compounds with 9 different types of atoms. The four generic datasets are: (1)Community: 500 two-community graphs with $60 \le |V| \le 160$. (2)Community-small: 500 two-community graphs with $12 \le |V| \le 20$. (3)Ego: 757 subgraphs extracted from Citeseer network[] with $50 \le |V| \le 399$.(4)Ego-small: 200 subgraphs extracted from Citeseer network with $4 \le |V| \le 18$ using random walk.

\textbf{Baselines.} We consider the following baselines: GraphRNN and GRAN ~\citep{you2018graphrnn,liao2019efficient} are autoregressive models. {GraphDF}~\citep{luo2021graphdf} is an autoregressive flow-based model. Moflow, GraphCNF \citep{zang2020moflow, lippe2020categorical} are flow-based models that generate graphs in one-shot. EDP-GNN and GDSS ~\citep{niu2020permutation,jo2022score} are one-shot score-based graph generative models. For molecule generation, we compare NVDiff with GraphDF, Moflow, GraphCNF, EDP-GNN, and GDSS. We compare generic graph generation with GraphRNN, GRAN, GraphCNF, EDP-GNN, and GDSS.

\textbf{Evaluation metrics.} We evaluate the generated molecules with the following metrics: {Validity} is the fraction of generated molecules that have valid chemical valency. 
{Novelty} and {Uniqueness} are the fraction of molecules not appearing in the training data and unique molecules, respectively. 
We evaluate the {Maximum Mean Discrepancy (MMD)} ~\citep{gretton2012kernel} between the test molecules and the generated molecules in terms of the {Neighborhood subgraph pairwise distance kernel (NSPDK)} ~\citep{costa2010fast}, which considers both structure and labels of the graph. 
{Fr\'echet ChemNet Distance (FCD)} ~\citep{preuer2018frechet} evaluates the diversity and the quality of the validly generated molecules by measuring the distance between feature vectors calculated for real and generated molecules. The FCD is arguably the most important metric since it captures the similarity between real and generated molecules' chemical properties. 
\scriptupdate{For the generated generic graphs, we evaluate the MMD distance between the test graphs and the generated graphs in terms of four type of graph features, including the statistics of degrees (Deg.), clustering coefficients (Clus.), and orbit counts (Orbit) from \citet{you2018graphrnn}, and the neural-based graph embedding (NN) proposed by \citet{thompson2022evaluation}.}
% For the generated generic graphs, following~\citet{you2018graphrnn}, we evaluate the MMD distance of the statistics of {degrees}, {clustering coefficients}, and {orbit counts} between the test graphs and the generated graphs. \scriptupdate{Besides, we also adopt neural based evaluation metric proposed by \citet{thompson2022evaluation}.} 
We report the metrics of the molecule and generic graph generation using 10000 and 128 samples, respectively.
% Uniqueness and Novelty are the percentage of unique molecules and molecules not appearing in the training data, respectively.
% We evaluate the model's performance on the molecular dataset with six metrics on the generated 10,000 samples. We report the percentage of the valid molecules and the proportion of unique molecules and measure the proportion of novelty molecules that did not appear in the training set. We also report FCD[], NSPDK[], and the likelihood.
% For generic datasets, we measure the Maximum Mean Discrepancy(MMD) for the degree, clustering coefficients, and occurrences of 4-node orbits. This metric is that the lower, the better.

% \begin{figure}
%     \centering
%     \begin{tabular}{cc}
%          \multicolumn{2}{c}{\includegraphics[width=0.96\textwidth]{figures/contextual.pdf}}\\
%          ~~~~~~~~~~Figure 2: Sampling speed~~~~~~~~~~ & Figure 3: Downstream task with contextual vector
%     \end{tabular}
%     % \includegraphics{}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

\input{tables/chemical-main}
\vspace{-1em}
\subsection{Quantitative Analysis}
\label{sec:exp-quan}
% v1
% Here we quantitatively estimate the quality of the generated graphs. Table 1 and Table 2 report the metrics evaluation on molecule generation and generic graph generation, respectively. 
Here we quantitatively estimate the quality of the generated molecules and generic graphs and report them in Table \ref{tab:molecule} and Table \ref{tab:generic}, respectively. \scriptupdate{We also analyze the sampling speed of NVDiff using the Ego dataset.}

% \textbf{Molecule Generation.} Molecules are relatively small and \textcolor{red}{their structures are much more complex (subtle?) than generic graphs}. We introduce NVDiff-E, a variant of NVDiff that generates both nodes and edges in the diffusion process for molecules. We observe that NVDiffs demonstrate their superior capability in generating valid molecules that share highly similar characteristics with the real molecules. Specifically, NVDiff and its variant significantly outperform all the baselines in terms of the FCD metric. We observe that NVDiff exhibits relatively lower validity and the highest FCD score on ZINC250K. \textcolor{red}{We argue that picking up the invalid molecules is easy as it can be checked via valency rule, while picking up the real ones is more difficult.} We also observe that the sampling speed is much faster than most baselines. Moreover, NVDiff achieves a comparable likelihood estimation to GraphCNF.

% v2
% {\red{
% \textbf{Molecule Generation.} Molecule Generation. We observe that NVDiff demonstrates it’s superior capability
% in generating valid molecules that share highly similar characteristics with the real molecules. Specifically, NVDiff significantly outperforms all the baselines in terms of the FCD metric. We observe that NVDiff exhibits relatively lower validity and the highest FCD score on ZINC250K. We argue that picking up the invalid molecules is easy as it can be done by checking valency rule, while picking up the real ones is more difficult. We also observe that the sampling speed is much faster than most baselines.}}

\textbf{Molecule generation.} NVDiff outperforms all baselines in terms of the FCD metric, thus superior in generating valid molecules that share highly similar characteristics with real molecules. However, on ZINC250K, we observe that NVDiff exhibits relatively lower validity. We argue that filtering invalid molecules is easy as it can be done by checking the valency rule while selecting realistic ones is difficult. We also observe that the sampling speed of NVDiff is much faster than most baselines.

\textbf{Generic graph generation.} We show the MMD evaluation on four datasets. Community and Ego contain massive nodes and thus are difficult to model by several baseline methods. We only report performance for baselines that converged in a reasonable time for these two datasets without consuming extensive computational resources. We observe that NVDiff outperforms all the baselines on most metrics. In GraphRNN, data are fit using BFS orderings, which are favored by datasets with community structure--the model naturally learns to generate communities sequentially. We argue that even without introducing such inductive bias, NVDiff still can capture the community pattern. In comparison, EDP-GNN and GraphCNF fail to capture the graph pattern of Community and Ego or exhibit poor performance on them. We hypothesize that the node-edge relationship becomes more complex as the graph size increases. So modeling nodes and edges in the diffusion prior is not a proper choice. Instead, the diffusion prior in NVDiff only needs to learn the node-to-node relationship, leaving the task of composing edges to the decoder.

\input{tables/common-main}

\textbf{Sampling speed.} Here we compared against other score-based graph generative models in terms of the sampling speed. \scriptupdate{We choose Ego for runtime analysis. Specifically, we manually fix the number of nodes the model will generate. For each setting, we sample 128 graphs and record the wall clock time. Figure \ref{tab:speed} shows the running time concerning the number of nodes of the generated graphs. NVDiff generates much faster than EDP-GNN and GDSS, especially over larger graphs.}
% \textbf{Sampling speed.} Here we compared against other score-based graph generative models in terms of the sampling speed. We choose Community for runtime analysis. Specifically, we manually fix the number of nodes the model will generate. For each setting, we sample 128 graphs and record the wall clock time. Figure \ref{tab:speed} shows the running time concerning the number of nodes of the generated graphs. NVDiff generates much faster than EDP-GNN, especially over larger graphs. Moreover, the running time of NVDiff increases linearly as the graphs' size increases, indicating the growth rate is constant with regard to graph size.

\begin{figure}
\begin{minipage}[b]{0.361\textwidth}
        \includegraphics[width=\textwidth]{figures/speed_ego.pdf} 
    \caption{\scriptupdate{Sampling speed}}
    \label{tab:speed}
\end{minipage}
\begin{minipage}[b]{0.564\textwidth}
        \includegraphics[width=\textwidth]{figures/contextual.pdf}
    \caption{Downstream tasks with contextual vector}
    \label{fig:context}
\end{minipage}
\vspace{-0.4cm}
\end{figure}
\vspace{-1em}
\subsection{Qualitative Analysis}

\label{sec:exp-qual}
We examine the effectiveness of NVDiff from three aspects: the denoising dynamics of node vectors, the graph statistics encoded in the contextual vector, and the quality of the generated molecules.

\begin{figure}
    \centering
    % \includegraphics[width=\textwidth]{figures/dynamic_v2.pdf}
    \includegraphics[width=\textwidth]{figures/dynamic_v2.pdf}
    \caption{Visualization of the denoising dynamics on Community dataset ({evolve from left to right}). Top row: t-SNE visualization over the node vectors, with color indicating the community membership. Bottom row: graphs generated from the corresponding node vectors via the decoder.}
    \label{fig:dynamic}
\end{figure}
\begin{figure}
    \small
    \centering
    \begin{tabular}{cccccc}
        &Reference &NVDiff & GraphDF & Moflow &  GraphCNF\\
        \rotatebox{90}{QM9}& 
        {\includegraphics[width=0.09\textwidth]{figures/sim/1185qm_ref.pdf}}& 
        {\includegraphics[width=0.17\textwidth]{figures/sim/1185qm.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1185qm_graphdf.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1185qm_moflow.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1185qm_graphcnf.pdf}}\\
      
     &  {\includegraphics[width=0.09\textwidth]{figures/sim/1193qm_ref.pdf}}& 
        {\includegraphics[width=0.17\textwidth]{figures/sim/1193qm.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1193qm_graphdf.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1193qm_moflow.pdf}}&
        {\includegraphics[width=0.17\textwidth]{figures/sim/1193qm_graphcnf.pdf}}\\
        \rotatebox{90}{ZINC250k}& {\includegraphics[width=0.09\textwidth]{figures/sim/1zinc_ref.pdf}}&
      {\includegraphics[width=0.17\textwidth]{figures/sim/1zinc.pdf}}&
     {\includegraphics[width=0.17\textwidth]{figures/sim/1zinc_graphdf.pdf}}&
      {\includegraphics[width=0.17\textwidth]{figures/sim/1zinc_moflow.pdf}}&
      {\includegraphics[width=0.17\textwidth]{figures/sim/1zinc_graphcnf.pdf}}\\
     &{\includegraphics[width=0.09\textwidth]{figures/sim/2zinc_ref.pdf}}& 
      {\includegraphics[width=0.17\textwidth]{figures/sim/2zinc.pdf}}&
     {\includegraphics[width=0.17\textwidth]{figures/sim/2zinc_graphdf.pdf}}&
      {\includegraphics[width=0.17\textwidth]{figures/sim/2zinc_moflow.pdf}}&
      {\includegraphics[width=0.17\textwidth]{figures/sim/2zinc_graphcnf.pdf}}\\
     
      \end{tabular}
      
    \caption{Molecule visualization with Tanimoto similarity. The left-most column visualizes the reference molecules randomly picked in the dataset. The top 2 molecules ranked by the similarity scores for each model are visualized. Extended results can be found in the Appendix \ref{app:extra-exp}.}
    \label{fig:mol_vis}
    \vspace{-0.6cm}
\end{figure}

\textbf{Denoising dynamics of node vectors.}
Figure \ref{fig:dynamic} shows how NVDiff generates node vectors and forms a community graph progressively. We record the node vectors along the denoising step. For each time step, we use t-SNE~\citep{van2008visualizing} to compress the node vectors for visualization. We color each node with its community membership obtained from the spectrum clustering. For each intermediate node vectors, we generate the graph using the learned decoder.
As the denoising step increases, node vectors from different communities become separable.% and the generated grap
% Unsurprisingly, our decoder fails to generate a community-like graph from node vectors where there arent sufficient structural information.

\textbf{Graph statistics in contextual vector.} We investigate whether the introduced contextual vector contains meaningful information about the graph, which can be used for supervising the diffusion process. Here we focus on QM9. We hypothesize that the contextual vector contains both the node and structural information. To validate this, we design three downstream tasks: atom type counting, cycle detection, and diameter prediction. The first task focuses on the global node statistics, and the last two tasks focus on the local and global structural contexts, respectively. We report accuracy for the cycle detection task and Mean Absolute Error (MAE) for the others. Figure \ref{fig:context} demonstrates the downstream task performance of the contextual vectors extracted from different time steps. We can observe that all task performance improves incrementally as time step decreases (i.e., node vectors get less noisy). Moreover, the predictions are precise when $t$ is close to $0$, indicating that the contextual vector encodes significant contexts locally and globally about the graph.
Interestingly, we find that the performance of tasks related to node context starts to converge earlier than those related to structural context. One reasonable explanation is that the node context is formed earlier than the structural context, as the latter usually depends on the former. We highlight the time step when the task starts to converge in the figure with a dash line. 


\textbf{Sample quality.} We inspect the drug-likeness of the generated samples by measuring the Tanimoto similarity of the Morgan fingerprint ~\citep{bajusz2015tanimoto}. Specifically, we calculate the pair-wise Tanimoto similarity between each generated sample and a real molecule randomly chosen from the dataset. Given a reference molecule, we retrieve the top 2 generated molecules ranked by the similarity score and visualize them in Figure \ref{fig:mol_vis}. We analyze samples generated from NVDiff, GraphDF, Moflow, and GraphCNF. Compared to other baselines, NVDiff can generate molecules that share a large substructure with the actual molecules, illustrating a superior modeling capability.

% \subsection{Sampling Speed \textcolor{red}{(quantitative)?}}
% Here we compared against other score-based graph generative model in terms of the sampling speed. We choose Community for runtime analysis. Specifically, we manually fix the number of nodes the model will generate. For each setting, we sample 128 graphs and record the wall clock time. Figure. \ref{tab:speed} shows the running time of the with regard to the number of nodes of the generated graphs. We observe that NVDiff generates much faster than EDP-GNN, especially over larger graphs. Moreover,the running time of NVDiff increases linearly as graphs' size increases, indicating the the growth rate is constant with regard to graph size.
% We report the performance on the molecule generation in Table. 1, and the performance on the generic graph generation in Table. 2.


% figure 1: sampling speed

% figure 2: visualization of graphs.

% table 3: validity on QM9 (the lower value is not because of overfit, instead is because the space is too small, this is proof by training on a small portion of the data, and then we have a high validity and 100\% novelty in the small training set but low novelty on the whole set)

% % \paragraph{Likelihood estimation through importance sampling}
% \begin{align}
% p(\bX,\bA) \approx	 \frac{1}{L}\sum_{l=1}^{L}\frac{p(\bX,\bA|\bZ^l)p(\bZ^l)}{q(\bZ^l|\bX,\bA)}; \bZ^l\sim q(\bZ|\bX,\bA)
% \end{align}

==> NIPS/sections/introduction.tex <==
\section{Introduction}\label{sec:intro}
% par1: Background [TODO: stuff about graph generation application]
% v1
% Graph generation is an important problem for various domains such as drug design and network modeling. This task remains to be challenging as it requires a generative model to describe the complex distribution of graph data, which are in a discrete and combinatorial space. Traditionally, graph data are described by simple graph distributions such Erdos-Renyi models, which often can only capture high-level statistics of the data. Recently,  graph generative models based neural networks are proposed to model fine-level graph structures and show promising results. 

Graph generation learns a distribution over graphs that helps summarize, predict, and explore various domains such as molecules and social networks~\citep{jin2018junction,watts1998collective}. This task is challenging because it requires a generative model to learn complex combinatorial patterns hidden in the graph data. One category of neural generative models sequentially generates nodes and edges of a graph~\citep{you2018graphrnn,liao2019efficient}. However, the generation probability of such a model varies when node ordering changes. Fitting such a model often requires node orderings, which often do not exist in training data. Furthermore, it is hard to train such models by maximizing the data likelihood \citep{chen2021order}. 

% v1
% Deep graph generative models mainly fall into two categories. The first type of models use autoregressive networks to generate entries of adjacency matrices [ref.]. These models  are not invariant to node permutations and require further technique to compute the likelihood of a graph []. The second type of models generate an adjacency matrix in one-shot[]. Early work such as VGAE first samples a group of node vectors independently from a multivariate Gaussian distribution, transforms them into latent node vectors with a neural network, and then generates an adjacency matrix from these vectors. VGAE is not flexible enough to generate high-quality graphs, though the main purpose of the model is to learn node vectors.  Later models assign latent vectors to both nodes and edges and then use more expressive models such as normalizing flows to describe the distribution of these vectors. 

% v1
% Recently Score-based generative models (SGMs) are used for one-shot graph generation. SGMs  are considered to be more flexible than normalizing flow models and have gained great success in generating realistic images. In graph domain, [] first propose to model the adjacency matrix of graphs using the framework of discrete-time SGM [], and introduce a novel noise conditional score network (NCSN), termed EDP-GNN. Based on this work, GDSS [] proposes to use two NCSNs to diffuse nodes and edges respectively. Furthermore, GDSS frames its models on the continuous-time domain to reduce sampling steps. Both models treat adjacency matrices as ``images'' and directly model these discrete matrices with diffusion processes.  

% v1
% All these recent generative models need to assign latent vectors to both nodes and edges. One research question is whether we can only model node vectors in the same way as VGAE. If we consider graph generation from the perspective of decomposing adjacency matrices, we can decide a sparse graph with a list of low-dimensional node vectors. The rigid Gaussian prior of VGAE is hard to sample vectors for nodes in a graph, but an SGM can be a flexible prior for sampling such vectors. A clear benefit of modeling node vectors only is the computational efficiency. It also helps to fight overfitting issues.

This paper focuses on another category of graph generative models, which assumes nodes are exchangeable~\citep{aldous1981representations,hoover1979}. Those models generate graphs as adjacency matrices invariant in probability when jointly shuffling rows and columns with a permutation $\pi$. There are two benefits to using exchangeable graphs. First, since node ordering does not affect the generation probability, calculating the likelihood of the graph only requires one pass with an arbitrary node ordering. Second, graph generation can be done in one-shot, i.e., parallel rather than sequential.

% v2
% The celebrated Aldous-Hoover theorem [] states that jointly exchangeable arrays can be represented as $A_{ij}\stackrel{d}{=}f(Z_i,Z_j,Z_{ij})$. Theoretically, $\mathbf{Z}=\{Z_i\}_{i\in[N]}\cup\{Z_{ij}\}_{(i,j)\in [N]^2}$ are uniform random variables representing hidden states of node $i,j$, and an edge between them. In practice, $Z$ can be finite-dimensional hidden vectors with any prior distribution. $f$ is a function encoding global and local context of the graph. Calculating likelihood is much easier for exchangeable graphs. When $\mathbf{Z}$ are conditional independent, graph generation can be executed in ``one-shot".

One early example of deep exchangeable graph generative models is VGAE ~\citep{kipf2016variational}. Based on the variational auto-encoder (VAE) freamwork~\cite{kingma2013auto}, VGAE represents the graph by latent node vectors. The priors of those latent vectors follow a multivariate Gaussian distribution, and they use an encoder to infer the variational posterior. VGAE uses an over-simplified prior and decoder. Its node vectors are independent, thus they cannot ``coordinate'' to play different roles in a meaningful graph.  

%thus suffering from posterior collapse problem~\citep{lucas2019understanding} when scaling up the decoder model, where the variational posterior collapse to the prior distribution. 

Recently, normalizing flows (NF)~\citep{rezende2015variational,liu2019graph,lippe2020categorical,xu2021learning} are introduced for graph generation by learning a reversible mapping from a Gaussian distribution to a continuous latent graph representation. However, the reversibility assumption restricts model design for NF models. For instance, graph normalizing flows (GNF)~\citep{liu2019graph} detaches NF with Graph Auto-Encoders, thus not guaranteed to maximize the overall likelihood. GraphCNF~\citep{lippe2020categorical} incorporates both node and edge latent vectors in NF and thus has a generative space with large dimensionality. 

%GraphCNF also sacrifices one-shot parallel generation to ensure exchangeability using a three-step generation.

% v2
% The flexibility of exchangeable graph models is determined by the decoder function $f$ and the distribution of $Z$. Oversimplified model design can be less expressive and harmful. A simple example is Erdos-Renyi model $G(n,p)$, where $f(\cdot,\cdot,\cdot)=p$ is a constant function capturing average edge occurrence probability without considering the personality of each node. Another example is VGAE [], which assumes $A_{ij}=1~\text{w.p.}~f(Z_i,Z_j)$, where $Z_i,Z_j$ are latent node vectors and $f$ is the decoder function. VGAE has two main drawbacks. First, it uses normal distribution as the prior, which is restricted and may suffer from posterior collapse problems. Second, VGAE does not capture the personality of each edge by removing edge vector $Z_{ij}$ from Aldos-Hoover's theorem. The inferior model choice makes  VGAE not flexible enough to generate high-quality graphs. Later models assign latent vectors to both nodes and edges and then use more expressive models such as normalizing flows to describe the distribution of these vectors. However, normalizing flows are still restrictive, since their network architectures are constrained to guarantee reversibility.

Score-based generative models (SGMs) introduce a diffusion process that maps observations into a noise distribution—reversing the diffusion process results in a generative model, which can be learned by score matching using, e.g., noise conditional score networks (NCSN)~\citep{song2019generative}. SGMs demonstrate superior performance than NF in generating realistic images and are recently adapted for one-shot graph generation. \citet{niu2020permutation} proposed EDP-GNN to model graphs using discrete-time SGMs. \citet{jo2022score} introduced GDSS, a continuous-time graph diffusion process for nodes and edges. Learning the graph generative process requires solving a system of reverse-time SDEs~\citep{anderson1982reverse,song2020score}. Both EDP-GNN and GDSS directly apply diffusion processes on edges. These methods are not scalable since their inference requires reversing a $\mathcal{O}(N^2)$-dimensional diffusion process. GDSS ignores the hierarchical interpretation between nodes and edges by modeling node and edge representations in parallel. %One research question is whether we can generate high-quality graphs from node vectors only if we use the expressive SGM as the prior of these vectors.

% v1
% In this work, we propose GraphLSGM, a novel generative model that models graphs in latent space via the framework of the score-based generative modeling. GraphLSGM takes a similar structure as VGAE but uses a highly flexible prior. One core component of the piror is the score network. Furthermore, we propose a attention-based NCSN for the purpose of graph diffusion, which attempts to capture both the global and the local information of a graph by introducing a contextual vector. Compared with models that use both node and edge vectors, our model is much more efficient in sampling and achieves comparable or better performance in graph generation tasks.  

In observation of those limitations, we propose NVDiff, a novel graph generative model built on latent score-based generative models (LSGM)~\citep{vahdat2021score}. The generative process first samples a latent representation of the graph and then decodes nodes and edges conditioning on the latent representation. In principle, the dimension of the latent space is arbitrary. To guarantee node exchangeability, we propose a diffusion process on latent node vectors, thus significantly reducing the dimension of the diffusion process from $\mathcal{O}(N^2)$ to $\mathcal{O}(N)$ and boosting sampling speed. Built on the NVDiff framework, we introduce an attention-based score network capturing local and global contexts within the graph by leveraging the self-attention mechanism with a contextual vector. NVDiff optimizes the variational lower bound of log-likelihood, which can be optimized end-to-end. Our empirical study demonstrates that NVDiff outperforms previous methods over various graph generation tasks. By diffusing only the node vectors, NVDiff can learn to generate larger graphs with high quality in one-shot. %\textcolor{red}{Moreover, we design various downstream tasks for the contextual vector in the proposed NCSN and show that it can encode significant graph statistics.}
% v1
% The contributions of this work are summarized as follows:
% \begin{itemize}
%     \item We propose node latent encoding strategy which allow us to characterize the graph distribution in a lower dimensional space and boost the sampling speed.
%     \item We propose a noise conditional score network for graph generation, leveraging the self-attention mechanism and graph neural network.
%     \item We achieve good performances in graph generation tasks.  
% \end{itemize}

The rest of the paper is organized as follows. In Section~\ref{sec:sgm} we review score-based generative models. Section~\ref{sec:nvdiff} introduces node vector diffusion models as a flexible graph generative process that preserve node exchangeability under the variational auto-encoder framework. Section~\ref{sec:related} reviews related works. We demonstrate that NVDiff achieves superior or comparable performance on multiple graph generation datasets with a significantly faster sampling speed in Section~\ref{sec:exp}. Section~\ref{sec:conclude} concludes.

% \begin{itemize}
%     \item We propose GraphLSGM, a score-based graph generative model which enjoys better expressivity and efficient sampling speed by introducing a latent variable framework.
%     \item \red{We introduce two major latent space encoding strategies -- one treats nodes as latent variables, and the other treats both nodes and edges as latent variables.}
%     % \item We propose to use node latent variables to encode all the structural and edge type information.
%     % in the consideration of model expressivity and model efficiency.
%     \item We propose a score network architecture that is suited for graph generation, by combining graph neural networks and self-attention mechanism.
% \end{itemize}

% \section{Introduction}
% % par1: Background [TODO: stuff about graph generation application]
% Graph generation tasks have broad applications in various domains, such as generating new molecules, modeling social relationships, and building knowledge graphs. This task remains to be very challenging as it requires capturing the complex distribution of the graph data, which is discrete and lies in a tremendously huge combinatorial space. Although many deep graph generative models have emerged, these models either need to depend on specific order and are hard to compute likelihood or cannot scale to large graphs.

% Deep graph generative models fall into two categories. One branch of them are deep autoregressive models[]. These models usually model graph data by capturing a sequence of decisions of adding nodes and edges, thus are unable to preserve the permutation-invariance property of $p(\bA)$, which requires further technique to compute the probability $p(G)$ of a graph. Other approaches seek to generate all nodes and edges in one-shot[]. Most of them are developed based on the framework of normalizing flow with coupling layers[]. Though admitting likelihood computation, it is unclear whether their expressive power are sufficient enough to capture all distributions[]. Besides, both of the autoregresssive models and flow-based models suffer from the scalability problem. The former needs to perform multiple decisions and the latter requires the dimensionality of the latent space to be identical to the data space.

% Score-based generative models (SGM) have gained great success in generating realistic images. In graph domain, [] first propose to model the adjacency matrix of graphs using the framework of discrete-time SGM [], and introduce a novel Noise Conditional Score Network (NCSN), termed EDP-GNN. Based on this work, GDSS [] proposes to use two NCSNs to diffuse nodes and edges respectively. Furthermore, GDSS frames its models on the continuous-time domain to reduce sampling steps. Though SGM is shown to be effective in graph generation problem, current approaches are still computationally expensive as they operate directly on data space and employ separate score networks for the data of two types, i.e., nodes and edges. Moreover, the expressive power of the employed NCSNs may be limited as the design choices are not fully investigated. 

% In this work, we propose GraphLSGM, a novel generative model that models graphs in latent space via the framework of the score-based generative modeling. To generate graphs, GraphLSGM first denoises samples drawn from the base distribution to the latent space, then maps the denoised latent embeddings to nodes and edges using a decoder. By carefully designing the latent space, we are able to improve the model expressivity [] as well as model efficiency. Furthermore, we propose a attention-based NCSN for the purpose of graph diffusion, which attempts to capture both the global information and the local information of a graph.

% Our empirical study indicates that [TODO experiment summary]. The contributions of this work are summarized as follows:
% \begin{itemize}
%     \item We propose GraphLSGM, a score-based graph generative model which enjoys better expressivity and efficient sampling speed by introducing a latent variable framework.
%     \item \red{We introduce two major latent space encoding strategies -- one treats nodes as latent variables, and the other treats both nodes and edges as latent variables.}
%     % \item We propose to use node latent variables to encode all the structural and edge type information.
%     % in the consideration of model expressivity and model efficiency.
%     \item We propose a score network architecture that is suited for graph generation, by combining graph neural networks and self-attention mechanism.
% \end{itemize}

==> NIPS/sections/methods.tex <==
\section{NVDiff: Graph Generation through Node Variable Diffusion} \label{sec:nvdiff}
% In this section, we use the VAE framework introduced above to model graph data. There are several issues to resolve before applying the LSGM to graph data.  We need to consider several issues: how to specify the prior  

% We first show our formulation of modeling graph in latent space in Sec. 3.1, leveraging the variational auto-encoder framework and the latent score-based generative model []. In Sec. 3.2, we introduce the parameterization of our VAE such that the structural information is maximally preserved in the latent space. We further discuss the architecture design of the proposed NSCN in Sec. 3.3. Finally, we present the training techniques and procedures for GraphLSGM in Sec. 3.4.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/ddgm-main.pdf}
\caption{In NVDiff, a graph $(\bA,\bX)$ is mapped to a set of latent node vectors $\bZ^0$ through an encoder, the joint distribution of the latent node vectors is model by a diffusion prior. To generate a graph, NVDiff first samples $\bZ^0$ by reversing the diffusion process, then generates nodes and edges by decoding the latent representation.}
\label{fig:framework}

\vspace{-1em}
\end{figure}
% \begin{figure*}
%     \centeriing
%     \includegraphics[width=100pt]{figures/ddgm-main.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure*}
\input{sections/methods/exchangeability}
\input{sections/methods/formulation}
\input{sections/methods/ncsn}
\input{sections/methods/vae}
\input{sections/methods/training}

% Let $\bZ^0=\bZ$, and $\bZ^1$ be the random variables with $p(\bZ^1)=\calN(\bZ^1|\mathbf{0}, \bI)$, the SGM prior can be described as 

% Denote $G=(\bX,\bA)$ to be a graph, where $\bX$ is the node attributes, and $\bA$ be all adjacency matrix with attribute. We further denote $K_v$ and $K_e$ to be the number of node type and the number of edge type, and $N$ be the number of nodes. Our goal is to model $p(G)$ by defining a exchangeable distribution $p(\bX,\bA)$.
% \begin{align}
%     p(G) = \frac{N!}{|\mathrm{Aut}(G)|}p(\bX,\bA)
% \end{align}
% we want to model $p(\bX,\bA)$ via a variational autoencoder
% \begin{align*}
%      \log{p(\bX,\bA)}\geq \mathcal{L}=\mathbb{E}_{q(\bZ|\bX,\bA)}\Big[\log{p(\bX, \bA,\bZ)} - \log{q(\bZ|\bX,\bA)}\Big]
% \end{align*}
% Here we denote $\bZ=(\bZ_v,\bZ_e)$, where $\bZ_v$ represent the latent variables of the node attributes, and $\bZ_e$ represents the latent variables of all possibles edges. Note that $\bZ_v$ is a $N\times K_v$ binary matrix, and $\bZ_e$ is a $(N\times N)\times (K_e+1)$ matrix, with an extra label denoting the class of non-edge. The ELBO $\mathcal{L}$ can be further written as 
% \begin{align}
%     \mathcal{L}(\theta,\phi,\psi,\bX,\bA)=&\mathbb{E}_{q_\phi(\bZ|\bX,\bA)}\Big[\log{p_{\theta,\psi}(\bX, \bA,\bZ)} - \log{q_\phi(\bZ|\bX,\bA)}\Big]\\
%     =&\mathbb{E}_{q_\phi}\Big[\log{p_\psi(\bX,\bA|\bZ)}\Big]
%     -\mathbb{E}_{q_\phi}\Big[\log{q_\phi(\bZ|\bX,\bA)}\Big]
%     +\mathbb{E}_{q_\phi}\Big[\log{p_\theta(\bZ)}\Big]
%     % =&\mathbb{E}_{q}\Big[\log{p(\bX,\bA|\bZ)}\Big]
%     % + \mathrm{KL}\Big(q(\bZ|\bX,\bA)||p(\bZ)\Big)
% \end{align}
% following LGSM \citep{vahdat2021score}, we denote the decoder parameter to be $\psi$, the encoder parameter to be $\phi$ and the learnable prior parameter to be $\theta$ we have the following formulation

% For the reconstruction term $\mathbb{E}_{q}\Big[\log{p(\bX,\bA|\bZ)}\Big]$, we have
% \begin{align*}
%     &\mathbb{E}_{q_\phi(\bZ|\bX,\bA)}\Big[\log{p_\psi(\bX,\bA|\bZ)}\Big]\\
%     =&\mathbb{E}_{q_\phi(\bZ|\bX,\bA)}\Big[\sum_{i=1}^n\log{p_\psi(\bX_i|\bZ_{v_{i}})}+\sum_{i=1}^{n}\sum_{j=1}^n\log{p_\psi(\bA_{i,j}|\bZ_{e_{i,j}})}\Big]
% \end{align*}
% When the prior is not learnable, we can use the reconstruction term and the KL term to compute the ELBO. This will be used to first pretrain the VAE without the diffusion process. We set the pre-fix prior $p(\bZ_\bX,\bZ_\bA)$ to be standard Normal. The KL term can be estimated without sampling from the encoder distribution, we omit the detail here. When the prior is learnable, we consider the equation 3. (We found that pretraining the VAE with fixed prior doesn't give a good reconstruction result, which we analyze the reason later)


% % For the entropy term $\mathbb{E}_{q}\Big[\log{q(\bZ|\bX,\bA)}\Big]$, we have
% % \begin{align*}
% %     &\mathbb{E}_{q_\phi(\bZ|\bX,\bA)}\Big[\log{q_\phi(\bZ|\bX,\bA)}\Big]\\
% %     =&\mathbb{E}_{q_\phi(\bZ|\bX,\bA)}\Big[\sum_{i=1}^n\log{q_\phi(\bZ_{v_i}|\bX, \bA)}+\sum_{i=1}^{n}\sum_{j=i+1}^n\log{q_\phi(\bZ_{A_{i,j}}|\bX, \bA)}\Big]
% % \end{align*}

% For the cross entropy term $\mathbb{E}_{q}\Big[\log{p(\bZ)}\Big]$, first we consider a diffusion process, let $\bZ=\bZ_0$, following LGSM, we have 
% \begin{align*}
%     &\mathbb{CE}\Big[q_\phi(\bZ_0|\bX,\bA)||p_\theta(\bZ_0)\Big]\\
%     =&\mathbb{E}_{t\sim\mathcal{U}(0,1)}\Big[\frac{w(t)}{2}\mathbb{E}_{q_\phi(\bZ_t,\bZ_0|\bX,\bA),\bm{\epsilon}}\big[||\bm{\epsilon}-\bm{\epsilon}_\theta(\bZ_t, t)||^2_2\big]\Big] + \frac{D}{2}\log{(2\pi e\sigma_0^2)}
% \end{align*}
% here $q_\phi(\bZ_t, \bZ_0|\bX,\bA)=q(\bZ_t|\bZ_0)q_\phi(\bZ_0|\bX,\bA)$, where the first term is defined as 
% \begin{align*}
%     q(\bZ_t|\bZ_0) = \mathcal{N}(\bm{\mu}_t(\bZ_0), \sigma_t)
% \end{align*}
% $q(\bZ_t|\bZ_0)$ is a Gaussian transition kernel that have a closed-form computation, to sample $\bZ_t$, we first draw $\bm{\epsilon}\sim\mathcal{N}(\bm{0},\bm{1})$, then let
% \begin{align*}
%     \bZ_t = \bm{\mu}_t(\bZ_0)+\sigma_t\bm{\bm{\epsilon}}
% \end{align*}
% $\mathcal{U}[0,1]$ denotes a uniform distribution that is used to draw time step $t$. $\sigma_0$ is defined as the to be the initial standard deviation for the encoder distribution, this value need to be defined to be as small as possible (check page 21 in the LSGM paper) and can not be 0 (can not integral over the distribution). Here we set $\sigma_0=0.001$. Another way is to set $\sigma_0=0$ and set the t sampling range to be $[\epsilon,1], \epsilon>0$. Note the $\sigma_0$ is used for the transition kernel, not for the encoder distribution $q_phi$

% For the second term the encoder distribution $q_\phi(\bZ_0|\bX,\bA)$. There are some considerations. As we are proposing to capture the joint distribution of the latent 
% \begin{align}
%     q_\phi(\bZ|\bX,\bA)=q_\phi(\bZ_v,\bZ_e|\bX,\bA)=q_\phi(\bZ_{v_1},\ldots,\bZ_{v_n},\bZ_{e_{1,1}},\ldots,\bZ_{e_{n,n}}|\bX,\bA)
% \end{align}
% Directly using mean-field and decompose the joint distribution to i.i.d standard normal variables wouldn't work, especially in molecular generation where atoms and bonds are highly correlated. However, complex distribution is hard to parameterized by a encoder. To circumvent this problem, we consider using normal distribution with small variance, in order to keep the correlation between different variables while obtaining the full supports in the latent space.
% \begin{align*}
%     q_\phi(\bX,\bA) = \mathcal{N}(\mu_\phi(\bX,\bA), \sigma^2_\phi(\bX,\bA)\bI)
% \end{align*}
% where the ideal value for $\sigma$ should be small. To achieve this we can fix it or add a regularization term.

==> NIPS/sections/methods/exchangeability.tex <==
\subsection{Graphs as Exchangeable Adjacency Matrices}
%Given an undirected graph $G$, calculating the likelihood for a sequentially graph generative model is hard, since it requires summing up all graph generation orders $\pi$: $p(G)=\sum_\pi p(G,\pi)$~\citep{you2018graphrnn,chen2021order}. On the other hand, calculating the likelihood of an exchangeable adjacency array is simple, since changing node ordering does not affect its generation probability. 

We consider an attributed graph $G$ with $N$ nodes and denote it by $(\bA, \bX)$. Here $\mathbf{A}\in\mathbb{R}^{N\times N\times K^e}$ denotes edge features, $\mathbf{X}\in\mathbb{R}^{N\times K^v}$ denotes node features, and feature dimensions are $K^e$ and $K^v$.
We mainly consider the case where nodes and edges are categorical data with one-hot vector representation. 

An exchangeable generative model $p$ requires $p(\mathbf{A},\mathbf{X})\stackrel{d}{=}p(\mathbf{A}[\pi,\pi,:],\mathbf{X}[\pi,:])$ for any permutation $\pi:[N]\rightarrow[N]$. $\mathbf{A}[\pi,\pi,:]$ represents the resulting matrix by jointly permuting the first and the second coordinates of $\mathbf{A}$, and $\mathbf{X}[\pi, :]$ represents permuting rows of $\mathbf{X}$ with $\pi$. With proper model design in the variational auto-encoder framework (VAE) by introducing intermediate latent variables, we can build flexible graph generative models without sacrificing exchangeability.


% v2
% For each $\pi$, there is an adjacency matrix $A$ corresponds to it. Exchangeable graphs assume the adjacency matrix is jointly exchangeable, i.e the probability of $A$ is invariant when shuffling its rows and columns with any permutation $\pi:[N]\rightarrow[N]$. The celebrated Aldous-Hoover theorem states that every binary exchangeable adjacency matrix has a representation formula.

% \begin{theorem}{\citep{aldous1981representations,hoover1979}}
% A random 2d-array $(A_{ij})_{i,j\in \mathbb{N}}$ is jointly
 %exchangeable if and only if there exists a random measurable function $f:[0,1]^3\rightarrow A$ such that $(A_{ij})\stackrel{d}{=} (f(Z_i,Z_j,Z_{ij}))$
% where $(Z_i)_{i\in \mathbb{N}}$ and $(Z_{ij})_{i,j>i\in\mathbb{N}}$ with $Z_{ij}=Z_{ji}$ are a sequence and matrix, respectively, of i.i.d. uniform $[0,1]$ random variables.
% \end{theorem}

% In Aldous-Hoover's representation, $Z_i$ and $Z_{ij}$ are latent variables that encode the property of each node and edge. In practice, modeling $Z_i$ and $Z_{ij}$ as conditional independent latent vectors will not break exchangeability. $f$ is a function encoding global and local context of the graph. The theorem is built on infinite-dimensional 2d-arrays, which applies to arbitrary finite-dimensional arrays as well.


==> NIPS/sections/methods/formulation.tex <==
\subsection{The VAE Framework}
\label{form}
% structure: vlb objective -> transforming the ce to score-matching -> diffusion prior needs to be perm-invariant.
Variational Graph Auto-Encoder (VGAE)~\cite{kipf2016variational} is a variational auto-encoder that models the distribution of adjacency matrices. It imposes a Gaussian prior $p(\bZ)$ over node vectors. During training, it maps $(\bA, \bX)$ to $\bZ$ using an encoder $q_{\phi}(\bZ | \bA , \bX)$ and then recover $\bA$ using a decoder $p_\psi(\bA | \bZ)$. 

%and generate the graph given $\bZ$ with .  %If we use an over-simplified prior such as $\mathcal{N}(\mathbf{0},\mathbf{I})$ and an expressive decoder, %VAE may suffers from posterior collapse problem. When this happens, the encoder passively converges to the prior, and the decoder is expressive enough to map the random noise (the prior) to the observation. 

Our work implements the VGAE framework and makes several important differences. (1) We use SGM as our prior $p_\theta(\bZ)$ to increase expressiveness. (2) We use decoder $p_\psi(\bA,\bX|\bZ)$ to model both nodes and edges. (3) We make adjustment to the encoder $q_\phi(\bZ | \bA, \bX)$ to facilitate model training. We highlight our framework in Figure \ref{fig:framework}.

Learning VAE requires maximizing the variational lower bound $\calL(\phi, \psi, \theta)$ of log-likelihood $\log{p(\bA,\bX)}$ as
\begin{align}
\max_{\phi, \psi, \theta}~\calL(\phi, \psi, \theta) \!= &\mathbb{E}_{q_\phi(\bZ|\bA,\bX)}\big[\log{p_{\psi}(\bA,\bX|\bZ)}\big] \!+\! \mathbb{E}_{q_\phi(\bZ|\bA,\bX)} \big[\log p_\theta(\bZ)\big]\!+\!\mathbb{H}\big[q_\phi(\bZ|\bA,\bX)\big]. \label{vlb}
\end{align}

In principle, $\bZ$ can be a latent variable with any dimension. Moderately compressed $\bZ$ enjoys compact representation and improves sampling speed of SGM. In NVDiff, we choose $\bZ \in \bbR^{N \times d}$, where each row corresponds to a latent node vector. To generate graphs, we first draw node vectors $\bZ\sim p_\theta(\bZ)$ and draw $\bA,\bX\sim p_{\psi}(\bA,\bX|\bZ)$. Edge information is encoded in mutually-dependent node vectors through a learnable SGM prior $p_\theta(\bZ)$. 


% In NVDiff, learning $p_\theta(\bZ)$ is equivalent to learning the score network $\epsilon_\theta(\bZ^{t}, t):\mathbb{R}^{N\times d}\times \mathbb{R}\rightarrow \mathbb{R}^{N\times d}$. To guarantee exchangeability of the SGM prior , $\epsilon_\theta(\bZ^{t}, t)$ needs to be permutation-equivariant in rows, i.e., $\epsilon_\theta(\bZ^t, t)[\pi,:] = \epsilon_\theta(\bZ^t[\pi,:], t)$ for any permutation $\pi$~\citep{niu2020permutation}.

% Below we design the NCSN, the decoder, and the encoder. 

% v1
% {In our problem, $(\bA, \bX)$ are observed, and we will introduce a latent variable $\bZ \in \bbR^{N \times d}$, each row of which is the latent vector for a node.
% In our VAE, the decoder is  $p_\psi(\bA, \bX | \bZ)$, and the encoder is $q_{\phi}(\bZ | \bA, \bX)$ -- they will instantiated latter. Then the variational lower bound $\calL(\bA, \bX; \psi, \phi, \theta)$ of log-likelihood $\log{p(\bA,\bX)}$ is 
% \begin{align}
% \calL(\bA, \bX; \psi, \phi, \theta) = &\mathbb{E}_{q_\phi(\bZ|\bA,\bX)}\Big[\log{p_{\psi}(\bA,\bX|\bZ)}\Big]-\mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p_\theta(\bZ)) \label{vlb}
% \end{align}
% The prior $p_\theta(\bZ)$is from the score-based diffusion model introduced in the previous section, and $\theta$ denotes its parameters.}

% v1
% {In the context of graph generation, the model first generate a set of node vectors $\bZ \sim p_\theta(\bZ)$ and them from a graph based on these vectors. Different VGAE models, node vectors from this distribution are not independent, so they are able to coordinate their roles in the graph. Different with models that also assign edge vectors, our model recover graph edges from node vectors only.}  


%%%%%%%%%%%%%%%%%%%%%
%The AISTATS paper already has a proof on this
%%%%%%%%%%%%%%%%%%%%%%%%
%Specifically, when the likelihood $p(\bA,\bX)$ is permutation-invariant, we require that the SGM prior $p_\theta(\bZ)$ is also permutation-invariant. We show:
%\begin{theorem}
%\label{th1}
%$p_\theta(\bZ^0)$ is permutation-invariant if the base distribution $p_1(\bZ^1)$ is permutation-invariant and, $\forall t\in[\Delta t,1]$, the reverse transition distribution $q(\bZ^{t-\Delta t}|\bZ^{t})$ is permutation-equivariant, i.e., $ p_\theta(\bZ^1)=p_\theta(\pi(\bZ^1))$ and $q(\bZ^{t-\Delta t}|\bZ^t)=q(\pi(\bZ^{t-\Delta t})|\pi(\bZ^t)) \rightarrow  p_\theta(\bZ^0)=p_\theta(\pi(\bZ^0)) $
%\end{theorem}
%By choosing the base distribution and transition distributions to be normal distributions, we shows that the SGM prior $p_\theta(\bZ)$ is permutation-invariant. \red{The formal proof of the theorem is presented in Appendix A}. Besides, the encoder distribution $q_\phi(\bZ|\bA,\bX)$ and the decoder distribution $p_\psi(\bA,\bX|\bZ)$ need to be permutation-equivariant in order to maintain permutation-invariant property of the likelihood [].
%
%%%%%%%%%%%%%%%%%%%%%%
%%The optimization should be in the section of parametering the prior. It seems that this part is known from the background section -- no innovation here, and we should put it to a position less important. 
%%%%%%%%%%%%%%%%%%%%%%
%Since we formulate $p_\theta(\bZ)$ into be a score-based model, in the objective above, the KL divergence $\mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p_\theta(\bZ))$ is not analytically accessible []. Instead, we can decompose it into the entropy of the approximate posterior and the cross entropy between the approximate posterior and the flexible prior. And for the cross entropy term, which involves the flexible prior, we substitute it with Eq. \eqref{ce-mse}. In our case, the rewritten cross entropy is:
%\begin{align}
%    \mathbb{CE}(q_\phi(\bZ^0|\bA,\bX)||p_\theta(\bZ^0))=\bbE_t\Big[\frac{g(t)^2}{2}\bbE_{q_\phi(\bZ^0,\bZ^t|\bA,\bX)}\big[||\nabla_{\bZ^t}\log{q(\bZ^t|\bZ^0)} - \bepsilon_\theta(\bZ^t)||^2_2\big]\Big] +\frac{C}{2} \label{ce-mse-graph}
%\end{align}
%where the constant $C=Nd\log{2\pi e\sigma^2_0}$, with a hyperparameter $\sigma_0$[], $\bZ^0=\bZ$ is the beginning of the prior diffusion process, and $\bZ^1\sim\calN(\bZ^1;\bzero, \bI)$ is the end of the diffusion process. Here, we set $q_\phi(\bZ^0,\bZ^t|\bA,\bX) = q_\phi(\bZ^0|\bA,\bX)q(\bZ^t|\bZ^0)$, with the forward transition kernel $q(\bZ^t|\bZ^0)=\calN(\bZ^t;\alpha_t\bZ^0,\sigma_t\bI)$, where
%$\alpha_t$ and $\sigma_t$ are computed based on time step $t$. 
%% \red{$\alpha_t=todo, \beta_t=todo$. Correspondingly, we have the reverse transition..}.
%


==> NIPS/sections/methods/ncsn.tex <==
\subsection{Attention-based Score Network with Contextual Embedding} \label{subsec:ncsn}
% v1
% The NCSN $\epsilon_\theta(\bZ^{t}, t)$ needs to predict the score vector $\bepsilon \in \bbR^{N \times d}$. There are several issues to consider in the design of the NCSN. First, it needs to be permutation-equivalent, that is, $\epsilon_\theta(\bZ^t, t) =  \epsilon_\theta(\bZ^t[\pi], t)$, for any permutation $\pi$. Second, unlike previous models, which often use a partially generated matrix to run a Graph Neural Network~(GNN), we need to model node vectors without any edge information. Third, the model needs to have a convenient way to express the global property of the graph to be generated. 

% By using a permutation equivalent NCSN, $p_\theta(\bZ)$ is guaranteed to be exchangeable~\citep{niu2020permutation}. In practice, we implement an attention-based NCSN capturing local and global contexts within the graph by leveraging the self-attention mechanism with contextual vector. 

% v2
% In NVDiff, learning the prior is equivalent to learning the score network $\epsilon_\theta(\bZ^{t}, t):\mathbb{R}^{N\times d}\times \mathbb{R}\rightarrow \mathbb{R}^{N\times d}$. There are two main considerations to design $\epsilon_\theta(\bZ^{t}, t)$. First, it needs to be permutation-equivalent, i.e. $\epsilon_\theta(\bZ^t, t) = \epsilon_\theta(\bZ^t[\pi,:], t)$ for any permutation $\pi$. We want the diffusion of node vectors to consider the global structure of the graph to be generated.

In NVDiff, learning $p_\theta(\bZ)$ is equivalent to learning the score network $\epsilon_\theta(\bZ^{t}, t):\mathbb{R}^{N\times d}\times \mathbb{R}\rightarrow \mathbb{R}^{N\times d}$. To guarantee exchangeability of the SGM prior , $\epsilon_\theta(\bZ^{t}, t)$ needs to be permutation-equivariant in rows, i.e., $\epsilon_\theta(\bZ^t, t)[\pi,:] = \epsilon_\theta(\bZ^t[\pi,:], t)$ for any permutation $\pi$~\citep{niu2020permutation}.


% v1
% {To guarantee permutation-equivalence, we use multi-head self-attention layers to construct the network. We first prepare the input to the network. Following~\citet{song2020score}. We encode $t$ to a vector $\bt$ with position encoding: $\bt = \mathrm{pe}(t)$. Then 
% \begin{align}
%     \bH_{0} = \mathrm{mlp}_{\mathrm{in}}([\bZ^t; \bone \bt^\top])
%     %\mbox{mlp}^{in}(\big[\bZ^t;\bH^t\big]),~\bH^t=\mbox{PE}(t)
% \end{align}
% Here $[\cdot; \cdot]$ concatenates rows of the two matrices, and the muli-layer perceptron $\mathrm{mlp}(\cdot)$ applies to rows of its argument. }

To guarantee permutation-equivariance without losing expressiveness, we use multi-head self-attention layers (MHA) to construct $\epsilon_\theta(\bZ^{t},t)$. Following~\citet{song2020score}, we transform $t$ to its positional encoding vector $\bt = \mathrm{pe}(t)$ as an input to the initial  mutli-layer perceptron (MLP) layer:
\begin{align}
    \bH_{0} = \mathrm{mlp}^{\mathrm{in}}([\bZ^t; \bone \bt^\top]),
    %\mbox{mlp}^{in}(\big[\bZ^t;\bH^t\big]),~\bH^t=\mbox{PE}(t)
\end{align}
where $[\cdot; \cdot]$ represents stacking two matrices by aligning their rows, and the $\mathrm{mlp}^\mathrm{in}(\cdot)$ applies to rows of its argument. 

% v1
% Then we stack $L$ multi-head attention layers (MHA) to process the input $\bH_0$. The innovation here is to reserve a global vector that allows the network to store global information about the graph. 
% \begin{align}
%     (\bg'_{\ell}, \bH_{\ell}) = \mbox{mha}([\bg_{\ell-1}; \bH_{\ell-1}]) , \quad
%     \bg_{\ell} = \bg_{\ell-1} + \bg'_{\ell}, 
%     \quad
%     \ell = 1,\ldots, L 
% \end{align}
% Here $\mathrm{mha}(\cdot)$ is a multi-head attention layer.  The global vector $\bg_{0}$ is initialized to a learnable vector. 

Then we stack $L$ MHA layers to process the input $\bH_0$ and incorporate a learnable global vector $\bg_{0}$ to carry graph information through MHA layers:
\begin{align}
    (\bg'_{\ell}, \bH_{\ell}) = \mathrm{mha}([\bg_{\ell-1}; \bH_{\ell-1}]) , \quad
    \bg_{\ell} = \bg_{\ell-1} + \bg'_{\ell}, 
    \quad
    \ell = 1,\ldots, L.
\end{align}

Finally, we predict the score from the representation $\bH_{L}$:
\begin{align}
    \hat{\bepsilon} = \mathrm{mlp}^{\mathrm{out}}(\bH_{L}).
\end{align}
% \red{bring up edge base a little}




% At each prediction, the contextual vector first summarizes the graph contexts by attending all nodes at $\ell=0$.

% v1
% \textcolor{red}{One may argue that $\bg_0$ has no information because it is the same for all graphs. However, the global vectors $\bg_\ell$ serves as a mailbox shared by all vectors in $\bZ^{t}$. In the generation process, a global vector can extract/distribute global information from/to node vectors to direct the formation of graph. The hypothesis is verified later in our experiments.}

% v2
% \red{re-write}
% For each denoising step in the generation process, given the noisy node vector $\bZ^t$, the contextual vector first extract the global information by attending all the node vectors at the first MHA layer. Once it encodes the graph context, there are two direction of information flows between the contextual vector and the node vectors: distributing graph context to guide node vector formations and \textcolor{red}{aggregating new graph context} from the node vector updates. \textcolor{red}{The NCSN iteratively runs such processes and obtain the evolution direction, i.e., the scores, which implicitly direct the formation of a graph.}

% The input of the score network $\bZ^t$ is a corrupted sample from the encoder, thus naturally carrying blurred global structural information. We use a contextual vector $\bg_0$ to carry the global information by attending all the node vectors at the first MHA layer. The following MHA layers gradually mix information between the contextual vector $\bg$ and the node vectors $\bH$ through self-attention until getting the output score.


\scriptupdate{The input of the score network $\bZ^t$ is sampled from a transition distribution $q(\bZ^t|\bZ^0)=\mathcal{N}(\bZ^t;\bmu_t(\bZ^0),\sigma_t\bI)$, which has a closed form with $\bmu_t(\cdot)$ and $\sigma_t$ determined by $t$. Since $\bZ^t$ naturally carries blurred structural information of each node, we use a contextual vector $\bg_0$ to carry the global information by attending all the node vectors at the first MHA layer.} The following MHA layers gradually mix information between the contextual vector $\bg$ and the node vectors $\bH$ through self-attention until getting the output score.

% v3
% \textcolor{red}{
% When we use the network to draw samples, we starts with $\bZ^1$ drawn from $N(\bzero, \bI)$ and use equation xx [please put a sampling equation in background] iteratively denoise it to eventually get $\bZ^0$, which is a sample $\bZ$ from the prior. 
% }

To draw a sample $\bZ^0$ from $p_\theta(\bZ)$, we first draw $\bZ^1$ from $\mathcal{N}(\bZ^1;\bzero, \bI)$ and run the reverse-time SDE (Eqn.~(\ref{reverse-sde})) with true score function $\nabla_{\bZ^t}\log{q_t(\bZ^t)}$ replaced by the score network $\epsilon_\theta(\bZ^{t},t)$~\citep{song2020score}.


% \subsection{Attention-based Score Network \red{(not revised yet)}}
% Our NCSN $\epsilon_\theta(\cdot, \cdot)$ takes in the noisy latent matrix $\bZ$, and the time step $t\in [0, 1]$, and predict the noise (score). First we define the input for the network:
% \begin{align}
%     \bH^{v,(0)} = \mbox{mlp}_v^{in}(\big[\bZ;\bH^t\big]),~\bH^{e,(0)} = \mbox{mlp}_e^{in}(\big[\bZ^e; \bH^t\big]),~\bH^t=\mbox{PE}(t)
% \end{align}
% where $\bH_t$ is the position embedding matrix output by $\mbox{PE}(\cdot)$ which takes time $t$ as input, and $\big[\cdot;\cdot\big]$ represents concatenate operation. While we do not have the edge features in the node latent space, we create the edge features $\bZ^e$ by computing the L2 distance between the nodes of the edge, for each $\bz^e_{ij}$ in $\bZ^e$, we have $\bz^e_{ij}=||\bz_i-\bz_j||^2_2$.

% We stack $L$ SFN layers to obtain the final node representation $\bH^{v}_{(L)}$, we defer the details of the SFN module, the following computations are repeated $L$ times:
% \begin{align}
%     (\bh^{ctx}_{(l)}, \bH^{v}_{(l)},\bH^{e}_{(l)}) = \mbox{SFN}(\bh^{ctx}_{(l-1)}, \bH^{v}_{(l-1)},\bH^{e}_{(l-1)})
% \end{align}
% here $\bh^{ctx}_{(0)}$, the input to the first SFN module, is a learnable context embedding in the score network. We predict the score from the final representations.
% % 
% \begin{align}
%     \hat{\epsilon} = \mbox{mlp}^{out}(\bH^{v}_{(L)})
% \end{align}

% \textbf{SFN.} Here we define SFN module. The SFN module is used for update the three given inputs $\bh^{ctx}$, $\bH^{v}$, and $\bH^{e}$, where $\bH^{v},\bH^{e}$ are the node hidden vectors and edge hidden vectors, respectively, and $\bh^{ctx}$ is the learnable context vector. 

% The SFN modules is composed as followed, we first update the node hidden vectors with a multi-head attention module (MHA), under the supervision of the context vector $\bh^{ctx}$. The context vector is assumed to contains the global information of the graph, and hence is able to put different semantic meaning (such as cluster or fragment membership) to the nodes. 
% \begin{align}
%     \hat{\bh}^{ctx}, \hat{\bH}_v &= \mbox{MHA}([\bh^{ctx};\bH^v])\\
%     \hat{\bh}^{ctx} &=  \hat{\bh}^{ctx}+\bh^{ctx}
% \end{align}
% Then we aggregate the edge features $\bh^e_{ij}$ into the node vectors $\hat{\bh}^v_{i}$, for node $i$, we first compute the message that passed from node $j$ to node $i$ through edge $e_{ij}$
% \begin{align}
%     {\mathbf{m}}_{ij} = \mbox{mlp}^m(\big[\mbox{mlp}^m_v(\hat{\bh}^v_{i});\mbox{mlp}^m_e(\bh^e_{ij});\mbox{mlp}^m_{ctx}(\hat{\bh}^{ctx})\big])
% \end{align}
% to aggregate message to node $v_i$, we first employ the attention mechanism to compute the message weight $w_{ij}$ following GAT,
% \begin{align}
%     w_{ij} = \frac{\mbox{exp}(\ba^T\big[\bW_v\hat{\bh}^v_{i}+\bW_v\hat{\bh}^v_{j};\bW_e\bh^e_{ij}\big])}{\sum_{j:j\neq i}\mbox{exp}(\ba^T\big[\bW_v\hat{\bh}^v_{i}+\bW_v\hat{\bh}^v_{j};\bW_e\bh^e_{ij}\big])}
% \end{align}
% here $\bW_v$ and $\bW_e$ are the learnable linear transform matrices for node vectors and edge vectors respectively, and $\ba$ is another learnable weight vector. We aggregate the messages into the node feature while maintaining the original information at the same time
% \begin{align}
%     \hat{\bh}^v_{i} = \hat{\bh}^v_{i} + \sum_{j:j\neq i} w_{ij}{\mathbf{m}}_{ij}
% \end{align}
% For edge updates, we apply the following operation to maintain the permutation equivariance.
% \begin{align}
%     \hat{\bh}^e_{ij} = \mbox{mlp}^e(\big[\bh^e_{ij};\mbox{mlp}^e_v(\hat{\bh}^v_{i})+\mbox{mlp}^e_v(\hat{\bh}^v_{j})\big])
% \end{align}

% \paragraph{Running time:} In GraphLSGM, two sampling steps are involved: (1) sampling $\bZ^0$ from $p_\theta(\bZ^0)$, which takes $T$ reversed diffusion steps to transform $\bZ^1$ to $\bZ^0$; and (2) transforming the sampled $\bZ^0$ to the graph. For diffusion frameworks that operate directly on data space, the time complexity is $O(TN^2)$, while for GraphLSGM, the time complexity is $O(TN+N^2)$. Note that we have $T\geq N$ in most cases, making $T$ a non-trivial constant.

==> NIPS/sections/methods/training.tex <==

\subsection{Training}
% v1
% In this section, we elaborate on the training objective of the GraphLSGM, and present a training algorithm that optimizes the parameters of VAE and the diffusion prior in a disjoint manner. We can further decompose the VLB objective $\calL(\theta,\phi,\psi,\bA,\bX)$ into:

In this section, we present the training procedure that iteratively optimizes the encoder, the decoder, and the diffusion prior. The training procedure is shown in Alg. \ref{alg}.  In the optimization objective $\calL(\phi,\psi,\theta)$ in Eqn.~(\ref{vlb}), the first term $\mathbb{E}_{q_\phi(\bZ|\bA,\bX)}\big[\log{p_{\psi}(\bA,\bX|\bZ)}\big]$ is the reconstruction term. We apply the reparameterization technique \citep{kingma2013auto} and use Monte Carlo samples to estimate the expectation.
% For training the VAE, we have the following objective:
% \underbrace{A=B}_{\text{Fermat}}
\citet{vahdat2021score} shows that the cross-entropy term can be calculated through score matching:
\begin{align}
  &\mathbb{E}_{q_\phi(\bZ|\bA,\bX)} \big[\log p_\theta(\bZ)\big] =  \bbE_{t,\bepsilon,q_\phi(\bZ^0,\bZ^t|\bA,\bX)}\Big[\frac{g(t)^2}{2}||\bepsilon - \bepsilon_\theta(\bZ^t,t)||^2_2\Big],\nonumber\\ 
&\mbox{with}~t\sim U[0,1],~\bepsilon\sim\mathcal{N}(\bepsilon;\bzero,\bI),~q_\phi(\bZ^0,\bZ^t|\bA,\bX)=q(\bZ^t|\bZ^0)q_\phi(\bZ^0|\bA,\bX).
\end{align}
Here $q(\bZ^t|\bZ^0)$ is a Gaussian transition kernel. The cross-entropy term is also estimated through Monte Carlo method. We describe the details of computing the cross-entropy term in Appendix \ref{app:ce}.
The entropy term $\bbH[q_\phi(\bZ|\bA,\bX)]$ in Eqn. (\ref{vlb}) is a constant because we fix the variance of the posterior distribution.  

% v1
% {In practice, three optimization problems occur when training VAE. \textcolor{red}{(i) Because in the reconstruction term, the edge distribution is decomposed into edge-existence and edge-type distributions. While we fit the edge-type distributions for all possible edges, most of them are ineffective, blurring the optimizing signal of the effective ones. (mentioned before?) (ii) At the starting stage of the optimization, where the diffusion prior is not well-optimized, the regularization from a half-baked diffusion prior might be harmful to training the VAE. (iii) We want the decoder to be robust to the diffusion error made by the diffusion prior during sampling.} We adopt three approaches to resolve these problems to improve VAE optimization. }

%The reconstruction term can be further decomposed to $\calL_{Rec}=\calL_{Node}+\calL_{Edge}$. The entropy $-\mathbb{E}_{q_\phi(\bZ|\bA,\bX)}[\log{q_\phi(\bZ|\bA,\bX)}]$ is a constant as we fix the encoder variance. \textcolor{red}{And  "The cross entropy can be optimized by score matching?" }

Recall that $\calL(\phi,\psi,\theta) \!=\! \mathbb{E}_{q_\phi(\bZ|\bA,\bX)}\big[\log{p_{\psi}(\bA,\bX|\bZ)}\big] \!+\! \operatorname{KL}(q_\phi(\bZ|\bA,\bX)||p_\theta(\bZ))$. We use KL annealing to dynamically balance optimization between the $\operatorname{KL}$ term and the rest objective functions during training. KL annealing effectively prevents the variational posterior from converging to a premature diffusion prior.


 Sampling novel and unique graphs requires the decoder to be robust  to noise in node vectors, since the diffusion prior may generate node vectors unseen during training. We introduce a consistency regularization term to encourage the decoder to generalize better, by adapting to a perturbed latent variable $\tilde{\bZ}$. We define:
 % We further perturb the latent sample $\bZ^0$ with a noise distribution $\calN(\tilde{\bepsilon};\bzero;\sigma_1\bI)$, we define
\begin{align}
    &\calL_\mathrm{Reg}\!\!=\!\!\bbE_{\tilde{\bepsilon}, q_\phi(\bZ|\bA,\bX)}\big[\!\!-\!\log{p_\psi(\bA,\bX|\tilde{\bZ})}\big], ~~\mbox{with}~ \tilde{\bepsilon}\!\sim\!\calN(\bzero,\sigma_1\bI),~\bZ\!\sim\! q_\phi(\bZ|\bA,\bX),~\tilde{\bZ}\!=\!\bZ+\tilde{\bepsilon}.
% &\mbox{with}~t'\sim U[0,\Delta t],~\bepsilon\sim\mathcal{N}(\bepsilon;\bzero,\bI),~q_\phi(\bZ^0,\tilde{\bZ}^{t'}|\bA,\bX)=q_t(\tilde{\bZ}^{t'}|\bZ^0)q_\phi(\bZ^0|\bA,\bX).
\end{align}
Here $\sigma_1$ is a hyperparameter. We replace the reconstruction term with $\calL_\mathrm{Reg}$ and finetune the decoder.
% \textcolor{red}{$\tilde{\bZ}^{t'}$ represents a perturbation from $\bZ^0$ with transition kernel $q_t(\tilde{\bZ}^{t'}|\bZ^0)$.}
% v1
% By doing so, we ask the decoder to be robust to the node vectors sampled near time step $[0,\Delta t]$ through the diffusion. 
% \textbf{Pretrain with fix prior.}


% \begin{algorithm}[t]
%   \caption{\textcolor{red}{Training Procedure for NVDiff}}
%   \label{alg:training_algorithm_graphrnn}
%   \begin{algorithmic}
%     \STATE {\bfseries Input:} Graph dataset $\mathcal{G}=\{(\bA_1,\bX_1),\ldots\}$, encoder $q_\phi$, decoder $p_\psi$, diffusion prior $p_\theta$, transition kernel $q_t$, diffusion coefficient $g(\cdot)$, $t$-sampling cutoff $\Delta t$, and KL annealing coefficient $\lambda$
%       \FOR{$(\bA,\bX) \in \calG$}
%         \STATE \textbf{[Optimization of encoder and decoder]}
%         \STATE ~~~~Draw $\bZ^0\sim q_\phi(\bZ|\bX,\bA)$, $t\sim U[0,1]$, $\bepsilon\sim\mathcal{N}(\bepsilon;\bzero,\bI)$, $\bZ^t\sim q_t(\bZ^t|\bZ^0)$
%         \STATE ~~~~Minimize loss $\mathcal{L}_{VAE}=-\log{p_\psi(\bA,\bX|\bZ^0)}+\frac{\lambda g(t)^2}{2}||\bepsilon-\bepsilon_\theta(\bZ^t,t)||^2_2$ over $\phi$ and $\psi$
%         \STATE \textbf{[Optimization of diffusion prior]}
%         \STATE ~~~~Minimize the SGM loss $\mathcal{L}_{SGM}=\frac{g(t)}{2}||\bepsilon-\bepsilon_\theta(\bZ^t,t)||^2_2$ over $\theta$
%         \STATE \textbf{[Regularization of decoder]}
%         \STATE ~~~~Draw $t'\sim U[0,\Delta t]$, $\bepsilon'\sim\mathcal{N}(\bepsilon;\bzero,\bI)$,$\tilde{\bZ}^{t'}\sim q_t(\tilde{\bZ}^{t'}|\bZ^0)$
%         \STATE ~~~~Minimize regularization term $\calL_{Reg}=-\log{p_\psi(\bA,\bX|\tilde{\bZ}^{t'})}$ over $\psi$
%       \ENDFOR
%   \end{algorithmic}
% \end{algorithm}

% Here we introduce a trick when optimizing the Equation 15. Since only the entry who's $A^b_{ij}=1$ is going to have the distribution $p(\hat{\bA}_{ij}|\bz_i, \bz_j)$. We use the weight $p_{ij}$ learned from Equation 14 to decide which entries get more training signal and which ones are not. Let $\psi$ be the parameter of generative distribution $p$ The objective of training the edge reconstruction becomes

% where detach() remove the gradient of the model and $\odot$ represents hadamard product. This term can be seen as a soft version of indicators indicate that whether the parameters of the corresponding entry need to be optimized or not. By using the teacher-forcing techniques, this term can be also replaced by the ground-truth binary adjacency matrix. (teacher-forcing turns out to be very necessary)

% the optimization of the parameters w.r.t the VAE poses two challenges
% The optimizations of the VAE and the diffusion prior are trained disjointly
% story line:
% 1. Optimization objectives w.r.t VAE and diffusion prior (instantiation of the LSGM objective)
% 2. VAE: KL annealing + the Decoder (teacher forcing)
% 3. algorithm (algo 2. in LSGM, need to specify the tricks we add to)

\begin{algorithm}[t]
  \caption{{Training Procedure for NVDiff}}
  \begin{algorithmic}
    \STATE {\bfseries Input:} Graph dataset $\mathcal{G}=\{(\bA_1,\bX_1),\ldots\}$, encoder $q_\phi$, encoder $p_\psi$, diffusion prior $p_\theta$, transition kernel $q$, diffusion coefficient $g(\cdot)$
      \FOR{$(\bA,\bX) \in \calG$}
        \STATE \textbf{[Optimize the encoder and the decoder]}
        \STATE ~~~~Draw $\bZ^0\sim q_\phi(\bZ|\bX,\bA)$, $t\sim U[0,1]$, $\bepsilon\sim\mathcal{N}(\bepsilon;\bzero,\bI)$, $\bZ^t\sim q(\bZ^t|\bZ^0)$.
        \STATE ~~~~Optimize $\mathcal{L}_\mathrm{VAE}=-\log{p_\psi(\bA,\bX|\bZ^0)}+\frac{ g(t)^2}{2}||\bepsilon-\bepsilon_\theta(\bZ^t,t)||^2_2$ over $\phi$ and $\psi$ with one step.
        \STATE \textbf{[Optimize the SGM prior]}
        \STATE ~~~~Optimize  $\mathcal{L}_\mathrm{SGM}=\frac{g(t)}{2}||\bepsilon-\bepsilon_\theta(\bZ^t,t)||^2_2$ over $\theta$ with one step.
      \ENDFOR
  \end{algorithmic}
  \label{alg}
\end{algorithm}

==> NIPS/sections/methods/vae.tex <==
\subsection{Graph Decoding}
The decoder predicts node attributes, edges, and edge attributes from node representations $\bZ$. 
% We first transform $\bZ$ to get a matrix $\bR \in \bbR^{N \times N \times d'}$ and a tensor $\bS \in \bbR^{N \times d''}$. 
% \textcolor{red}{We first transform $\bZ$ to get the node logits $\bS \in \bbR^{N \times d'}$ and the edge logits $\bR \in \bbR^{N \times N \times d''}$. }
We first transform $\bZ$ to get the node representation $\bS \in \bbR^{N \times d'}$ and the edge representation $\bR \in \bbR^{N \times N \times d''}$ from the penultimate layer of the decoder.
\begin{align}
(\bS, \bR) = \mathrm{gnn}_{\psi}(\bZ, \bE), \quad \bE = [(\bz_i - \bz_j)^2: i, j = 1, \ldots, N].
\end{align}
Here $\bE\in\bbR^{N\times N\times d}$ is a tensor, whose $(i,j)$-th vector slice denotes the element-wise squared difference between two node vectors $\bz_i$ and $\bz_j$.
$\mathrm{gnn}_\psi(\cdot,\cdot)$ is a $M$-layer graph neural network that computes on a fully-connected graph with $\bZ,\bE$ being the node and edge inputs. The $\ell$-th layer of the GNN updates nodes and edges from $(\bS^{\ell-1},\bR^{\ell-1})$ to $(\bS^{\ell},\bR^{\ell})$ as follow: 
\begin{align}
    \br_{i,j}^{\ell}= \mathrm{mlp}^e([\bW^{e}\bs_{i}^{\ell-1} + \bW^e\bs_{j}^{\ell-1};\br_{i,j}^{\ell-1}]),\quad
    \bs_{i}^{\ell}= \mathrm{mlp}^v\Big(\Big[\sum_{j:j\neq i}^{N}\bW^{v}\br_{i,j}^{\ell};\bs_{i}^{\ell-1}\Big]\Big).
\end{align}
Here $\bs_i^\ell$ is the $i$-th row in $\bS^\ell$, $\br_{i,j}^\ell$ is the $(i,j)$-th vector slice in $\bR^\ell$,  we denote $(\bS^0,\bR^0):=(\bZ,\bE)$ as inputs to the GNN, and $(\bS,\bR):=(\bS^M,\bR^M)$. We recover node features and edge features respectively:
\begin{align}
p(\bA, \bX | \bZ) = p(\bA | \bR) p(\bX | \bS) = \prod_{i = 1}^{N} p(\bx_i | \bs_i) \prod_{j < i}  p(\ba_{i,j} | \br_{i,j}) ,
\end{align}
% Here $\ba_{i,j}$ and $\br_{i,j}$ are a fiber of $\bA$ and $\bR$ respectively; and $\bx_i$ and $\bs_i$ are a row of $\bX$ and $\bS$ respectively. 
where $\bx_i$ denotes the $i$-th row in $\bX$ and $\ba_{i,j}$ denotes the $(i,j)$-th vector slice in $\bA$. Since the adjacency matrix is symmetric, we consider the lower triangle only.   

Now we are ready to recover individual features for edges and nodes. When we consider an edge feature, we treat a non-edge ($\ba_{i,j} = \bzero$) separately from an actual edge label. 
We specify $p(\ba_{i,j} | \br_{i,j})$ with two set of probabilities:  
\begin{align} 
p(\ba_{i,j} = \bzero | \br_{i,j}) &= \mathrm{mlp}^b_{\psi}(\br_{i,j}), \\
p(\ba_{i,j}  | \ba_{i,j} \neq \bzero,  \br_{i,j}) &= \mathrm{Categorical}(\ba_{i,j}; \mathrm{mlp}^e_{\psi}(\br_{i,j})).
\end{align} 
Here $\mathrm{mlp}^b_{\psi}(\cdot)$ calculates the Bernoulli probability of the non-existence of edge $(i,j)$, and $\mathrm{mlp}^e_{\psi}(\cdot)$ calculates the categorical probabilities for the label of edge $(i,j)$. 


%%%%%%%%%%%%%
Then we consider node features and define:
\begin{align}
p(\bx_i | \bs_i) = \mathrm{Categorical}(\bx_i; \mathrm{mlp}^n_{\psi}(\bs_i)).
\end{align}
Here $\mathrm{mlp}^n_{\psi}(\cdot)$ is applied to get the probabilities of the categorical distribution. We use sigmoid activation function in the last layer of $\mathrm{mlp}^b_\psi(\cdot)$ and softmax activation function in the last layer of $\mathrm{mlp}^e_\psi(\cdot)$ and $\mathrm{mlp}^n_\psi(\cdot)$.

% \begin{align}
%     &p_\psi(\bA,\bX|\bZ)=p(\bX|\bR^v)p(\bA|\bR^e)=\prod_{i=1}^{N}p_\psi(\bx_i|\br^v_i)\prod_{i=1}^{N-1}\prod_{j=i+1}^{N}p_\psi(\ba_{ij}|\br^e_{ij})\\
%     &\mbox{with}~\bR^v=[\br^v_1;\ldots;\br_N^v],~~\bR^e=[\br^e_{12};\br^e_{13};\ldots;\br^e_{N-1,N}],~~(\bR^v,\bR^e)=\mbox{gnn}_\psi(\bZ,\bE)
% \end{align}


% and $\ba_{ij}$ to be the $(i,j)$-th entry of adjacency matrix $\bA$. We formulate decoder distribution $p_\psi(\bA,\bX|\bZ)$ as follow:



% v1
% where $q_\psi(\bx_i|\br^v_i)$ and $q_\psi(\ba_{ij}|\br^e_{ij})$ are categorical distributions over nodes and edges, respectively. $\bE=[\be_{12};\be_{13};\ldots;\be_{NN}]$ are the edge features with $\be_{ij}=||\bz_i-\bz_j||^2$. \textcolor{red}{We parameterize  $\mbox{gnn}_\psi(\cdot,\cdot)$ with a GNN ($M$-layer GCN?) that computes on a fully connected graph.} We update nodes and edges for each graph convolution layer as follows: 
%where $q_\psi(\bx_i|\br^v_i)$ and $q_\psi(\ba_{ij}|\br^e_{ij})$ are categorical distributions over nodes and edges, respectively. 


%Here we denote $(\bR^v_0,\bR^e_0):=(\bZ,\bE)$ as inputs to the GNN, and $(\bR^v,\bR^e):=(\bR^v_M,\bR^e_M)$ as GNN output hidden vectors. Given GNN outputs, we decode the node distribution as:
%\begin{align}
%    p_\psi(\bx_i|\br_i^v)=\mbox{Cat}(\bx_i|\gamma_{i,0},\ldots,\gamma_{i,K^v}),~~ \mbox{with}~(\gamma_{i,0},\ldots,\gamma_{i,K^v})=\mbox{mlp}(\br_i^v).
%\end{align}


%Since non-edge dominates other edge types in number, we decouple the edge decoder $p_\psi(\ba_{ij}|\br^e_{ij})$ to model edge-existence and edge-type separately to get rid of the class imbalance issue:
%\begin{align}
%    &p_\psi(\bb_{ij}|\br_{ij}^e) = \mbox{Bern}(\bb_{ij};p_{ij}),~ p_\psi(\bc_{ij}|\br_{ij}^e) = \mbox{Cat}(\bc_{ij};\eta_{ij,0}, \eta_{ij,1},\ldots, \eta_{ij, K^e})\\
%    &\mbox{where}~ (p_{ij}, \eta_{ij,0}, \eta_{ij,1},\ldots, \eta_{ij, K^e}) = f_\psi(
%\br^e_{ij}).
%\end{align}
%Here $\bb_{ij}$ is the binary variable indicating the possibility of the existence of an edge, $\bc_{ij}$ is the categorical variable indicating the edge type, with the $0$-th class being the non-edge type. We formulate $p_\psi(\ba_{ij}|\bh^e_{ij})$ by composing these two distributions:
%\begin{align}
%    &p_\psi(\ba_{ij}|\br_{ij}^e)=p_\psi(\ba_{ij}|\bb_{ij},\bc_{ij})=\mbox{Cat}(\ba_{ij};1-p_{ij}+p_{ij}\eta_{ij,0}, p_{ij}\eta_{ij,1},\ldots, p_{ij}\eta_{ij, K^e})
%\end{align}
% In doing so, the distribution is dominated by the edge-existence distribution $p_\psi(\bb_{ij}|\br_{ij}^e)$ such that the edge-type distribution $p_\psi(\bc_{ij}|\br_{ij}^e)$ is effective only when the possibility of forming an edge is high. We assume that $p_\psi(\bb_{ij}|\br_{ij}^e)$ and $p_\psi(\bc_{ij}|\br_{ij}^e)$ are independent given $\br_{ij}^e$, and optimize them separately.

% \red{re-write:}

% One non-trivial challenge is to parameterize the edge decoding distribution $p_\psi(\ba_{ij}|\br^e_{ij})$, which needs to model both the edge existence and the edge type.

% \red{should we show how to address the diffusion prior mismatch issue by making the decoder more robust here?}
%  We use the same notation that $K_e$ denotes the number of edge types. The task of decoding edge and edge type together turns to fitting a categorical distribution with $K_e+1$ class. Let $A$ be the adjacency matrix, given the node representation of node $i$ and node $j$, the distribution is show as follow
% \begin{align}
%     p(\bA_{ij}|\bZ_{v_i}, \bZ_{v_j}) = \mbox{Cat}(\pi_{ij,0}, \pi_{ij,1},\ldots, \pi_{ij, K_e})
% \end{align}
% \textbf{We find that fitting such distribution is difficult, i.e., the loss did not converge well. We propose another scheme for fitting the distribution}
% \begin{align}
%     p(\bA_{ij}|\bZ_{v_i}, \bZ_{v_j}) = P(\bA_{ij}|\bA_{ij}^b,\bZ_{v_i}, \bZ_{v_j})P(\bA_{ij}^b|\bZ_{v_i}, \bZ_{v_j})
% \end{align}
% where the $\bA_{ij}^b$ is bernoulli random variable that indicates the edge exists or not, without considering the edge feature. We introduce a proxy distribution $ p(\hat{\bA}_{ij}|\bz_i, \bz_j)$, and show
% \begin{align}
%     p(\bA_{ij}^b|\bZ_{v_i}, \bZ_{v_j}) &= \mbox{Bern}(p_{ij}|\bZ_{v_i}, \bZ_{v_j})\\
%     p(\hat{\bA}_{ij}|\bZ_{v_i}, \bZ_{v_j}) &=  \mbox{Cat}(\pi_{ij,0}, \pi_{ij,1},\ldots, \pi_{ij, K_e})\\
%     p(\bA_{ij}|\bZ_{v_i}, \bZ_{v_j})&=p(\bA_{ij}|\bA_{ij}^b,\hat{\bA}_{ij})=\mbox{Cat}(1-p_{ij}+p_{ij}\pi_{ij,0}, p_{ij}\pi_{ij,1},\ldots, p_{ij}\pi_{ij, K_e})
% \end{align}
% where $\pi_{ij,0}$ always stand for the class of the non-edge, we can easily show that the Equation 16 is also a valid categorical distribution. And ideally we want $\pi_{ij,0}$ is as smaller as possible. In optimization, we can directly optimize Equation 14 and 15. In equation 15, we can either optimize $\pi_{ij,0}$ or set it to close to 0 and just optimize the others.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Graph Encoding}

We use a mean-field distribution as   the encoder and parameterize it with a GNN:
\begin{align}
    q_\phi(\bZ|\bA,\bX) = \calN(\bZ; \bM, \sigma^2 \bI), \quad \bM = \mathrm{gnn}_\phi(\bA, \bX).
    % ;~ q_\phi(\bz_i|\bA,\bX)=\calN(\bz_i;\bmu_i,\bsigma_i\bI)
\end{align}
Here the encoder is a Gaussian distribution, whose mean is computed from a GNN. The architecture details are described in Appendix \ref{app:arch-enc}. To simplify the optimization objective, we fix the variance of the encoder and only optimize its mean parameters. 
% We can afford doing so because our prior is very flexible.
% v2
% \red{re-write}:
% Here we fix the variance of the encoder such that it only needs to model the mean of the normal distribution. 
By doing so, we constrain flexibility of the encoder and encourage the SGM prior to match the aggregated posterior.
When we apply a GNN to $(\bA, \bX)$, we treat non-edges as an extra edge-type and also pass messages through them. Following \citet{satorras2021n}, we also inject random noise to each node to break the symmetry of the graph such that nodes are separable. We find these measures improve the model performance. 
% distinguishable from each others.

% \textcolor{red}{With the introduced learnable diffusion prior, we fix the variance of the encoding distribution to constrain its flexibility such that the complexity of modeling a distribution is moved to the prior.}



%, \red{the details of the architecture is in the Appendix B.}

% We define the index-code mutual information within a graph as follow:
% \begin{align}
%   \mathbb{I}_{q(i;\bz|\bA,\bX)}(i;\bz|\bA,\bX)=\mathrm{KL}(q_\phi(i|\bz;\bX,\bA)||p_\theta(i|\bz))
% \end{align}
% Here we discuss the relation between the diffusion prior and the encoding distribution from the perspective of optimization.
% We first define the index of the node $i$ to be a random variable that depends on its corresponding graph $G$, and let $q(i|\bA,\bX)=1/N$. 
% For the diffusion prior, we consider that the $q_\theta(\bz)$ is actually learning to match the aggregated posterior $q_\phi(\bz)=\mathbb{E}_{p_{data}(\bA,\bX)}\mathbb{E}_{q(i|\bA,\bX)}[q_\phi(\bz_i|\bA,\bX)]$. For each posterior distribution $q_\phi(\bz_i|\bA,\bX)$, the KL term $\mathrm{KL}(q_\phi(\bz_i|\bA,\bX)||p_\theta(\bz_i))$ acts as a regularizer that enforces the encoder to place some appropriate ``overlap'' in the latent space and at the same time, makes the aggregating posterior $q_\phi(\bz)$ to match the diffusion prior. However, for graph latent models, we make the following observation:

% \begin{observation}
% A precise reconstruction of $(\bA,\bX)$ requires that  within the graph, for any node pairs $(i,j)$, the encoding distributions of node $i$ and node $j$ do not have significant overlap.
% \end{observation}
% Because if two nodes within a graph are decoded into two distributions that are similar to each other, the decoder is unable to distinguish which samples are drawn from which distribution, thus dampen the reconstruction quality. This problem is more severe when the \textit{posterior collapse} happens in our model, i.e., the encoding distributions collapse towards the diffusion prior for some graph $(\bA,\bX)$. To alleviate this issue, we fix the standard derivation of the encoding distribution to a tunable hyperparameter [CV-VAE, 1911.02469]. Empirically, we observe that the learned diffusion prior is closed to the aggregated posterior, and sampled latent variables can perfectly recover the graph.
% \begin{observation}
% The variance of the aggregated posterior $q_\phi(\bz)$ is relatively large compared to a single encoding distribution, so does the complex diffusion prior $p_\theta(\bz)$.
% \end{observation}





% Here we argue that in GraphLSGM, posterior collapse problem in the VAE is severe. As each 
% Derivation ($q(i)=1/N$):
% \begin{align*}
%     \mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p(\bZ)) &= -\mathbb{E}_{q(\bZ|\bA,\bX)}\big[\log{q(\bZ|\bA,\bX)}\big] + \mathbb{E}_{q(\bZ|\bA,\bX)}\big[\log{p(\bZ)}\big]\\
%     % &=\mathbb{E}_{q(\bz_1,\ldots,\bz_N|\bA,\bX)}\big[\sum_{i=1}^N\log{q(\bz_i|\bA,\bX)}\big]-\mathbb{E}_{q(\bz_1,\ldots,\bz_N|\bA,\bX)}\big[\sum_{i=1}^N\log{p(\bz_i)}\big]\\
%     % &= \sum_{i=1}^N\mathbb{E}_{q(\bz_i|\bA,\bX)}\big[\log{q(\bz_i|\bA,\bX)}\big] - \sum_{i=1}^N\mathbb{E}_{q(\bz_i|\bA,\bX)}\big[\log{p(\bz_i)}\big]\\
%     % &= \sum_{i=1}^N\mathbb{E}_{q(\bz|i,\bA,\bX)}\big[\log{q(\bz|i,\bA,\bX)}\big] - \sum_{i=1}^N\mathbb{E}_{q(\bz|i,\bA,\bX)}\big[\log{p(\bz)}\big]\\
%     &=N\mathbb{E}_{q(i)}\mathbb{E}_{q(\bz|i,\bA,\bX)}\big[\log{q(\bz|i,\bA,\bX)}\big] - N\mathbb{E}_{q(i)}\mathbb{E}_{q(\bz|i,\bA,\bX)}\big[\log{p(\bz)}\big]\\
%     &=N\mathbb{I}\big(\bz;i|\bA,\bX \big) +N \mathrm{KL}(q(\bz|\bA,\bX)||p(\bz))
%     % &=N\mathbb{E}_{q(\bz,i|\bA,\bX)}\big[\log{q(\bz|i,\bA,\bX)}\big] - N\mathbb{E}_{q(\bz|\bA,\bX)}\big[\log{p(\bz)}\big]\\
%     % &=N\mathbb{E}_{q(\bz,i|\bA,\bX)}\big[\log{\frac{q(\bz|i,\bA,\bX)q(i)q(\bz|\bA,\bX)}{q(i)q(\bz|\bA,\bX)}}\big] - N\mathbb{E}_{q(\bz|\bA,\bX)}\big[\log{p(\bz)}\big]\\
%     % &=\mathbb{E}_{q(\bz,i|\bA,\bX)}\big[\log{\frac{q(\bz,i|\bA,\bX)}{q(i)q(\bz|\bA,\bX)}}\big] +N\mathbb{E}_{q(\bz,i|\bA,\bX)}\big[\log{q(\bz|\bA,\bX)}\big]- N\mathbb{E}_{q(\bz|\bA,\bX)}\big[\log{p(\bz)}\big]\\
% \end{align*}
% To ease the training procedure of the diffusion prior, following [LSGM], we first pretrain our VAE model with a standard normal prior such that the diffusion prior only needs to model the mismatch between the aggregated posterior and the fixed prior. In GraphLSGM, each graph is represented by $N$ latent variables, and we wish the aggregated posterior can maximally match the fixed prior while the reconstruction recovered from the latent embeddings is precise. Note that we consider the aggregated posterior over $N$ nodes given an input, instead of all the observations in dataset. The reason behind this is that nodes within a graph should be separable and nodes from different graphs can share similar encoding distribution. Given a graph $G=(\bA,\bX)$, we rewrite the KL term as follow
% \begin{align}
%     % \mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p_\theta(\bZ))=\sum_{i=1}^{N}\mathbb{E}_{q_\phi(\bZ_i|\bA,\bX)}\Big[\log{q_\phi(\bZ_i|\bA,\bX)}-\log{p(\bZ_i)}\Big]
%     % \mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p_\theta(\bZ))=\sum_{i=1}^N\mathrm{CE}(q_\phi(\bz_i|\bA,\bX)|p(\bz_i))-\sum_{i=1}^N\mathbb{H}\big[q_\phi(\bz_i|\bA,\bX)\big]
%     \mathrm{KL}(q_\phi(\bZ|\bA,\bX)||p(\bZ))
%     &=N\mathbb{CE}(q_\phi(\bz|\bA,\bX)|p(\bz))-\sum_{i=1}^N\mathbb{H}\big[q_\phi(\bz_i|\bA,\bX)\big]
% \end{align}
% \red{where $\mathbb{CE}(q_\phi(\bz|\bA,\bX)|p(\bz))$ is the cross entropy between the aggregated posterior over $N$ nodes and the given prior, $\mathbb{H}\big[q_\phi(\bz_i|\bA,\bX)\big]$ is the entropy for the $i$-th node in the graph. (PS. the second term may be further simplified?}
% Intuitively, the KL term can be viewed as a regularizer in two aspects. The first term which involves the prior helps shape the latent space, and the second term prevents the encoding distributions from overfitting by enforcing overlap for different nodes. However, the entropy term $\mathbb{H}\big[q_\phi(\bz_i|\bA,\bX)\big]$ might impose unwanted effect on our task as it might cause nodes to be indistinguishable from each others, yielding a poor reconstruction result. Particularly, we find that during training, the optimizer finds it difficult to balance between giving a good reconstruction and placing certain amount of support to each encoding distribution. As the reconstruction performance is directly relative to the sample quality, we fix the entropy to a constant for all nodes such that the encoder and decoder can focus more on the reconstruction. This is equivalent to setting the variance of the encoder distribution to be a tunable hyperparameter [CV-VAE]. Empirically, we observe that the aggregated posterior $q_\phi(\bz|\bA,\bX)$ is closed to the fixed prior, and sampled latent variables can perfectly recover the graph. \red{todo: extend the joint-training a little bit} We adopt the same configuration when jointly training the VAE and the diffusion prior.



% we only need that inside a graph, nodes are separable 
% Specifically, we want 

% However, during training, such trade-off is found hard to balanced as the latter one tries to push all the node representations away from the zero-center such that they are distinguishable from each other. 

% potentially unwanted regularization effect from the KL term 



% However, since we have $N$ latent variables for each input $(\bA,\bX)$, 

% such pretraining scheme 
% Here we elaborate on the challenges for the encoder and the decoder separately and propose the solutions to them. 
% \paragraph{Encoder} 
% 1. the aggregated posterior $q(z)$ is closed to standard normal
% 2. the encoding distribution for each node $q(z_i|X,A)$ is distinguishable for each other, i.e., no significant overlap.

% $q_\phi(\bZ|\bA,\bX)$


==> NIPS/sections/preliminaries.tex <==
\section{Background: Score-based Generative Models}\label{sec:sgm}

% v1
%{\subsection{Graph Generative Modeling via Maximum Likelihood Estimation}
%We consider undirected graphs with node and edge features. For a graph $G$, we denote it with $N$ nodes, we denote its node features by a matrix $\bX\in\mathbb{R}^{N\times K^v}$ and its edge features by a tensor $\bA\in\mathbb{R}^{N\times N\times K^e}$. Here $K^v,K^e$ are respectively the dimensions of node features and edge features. The aim of this work is to define a distribution $p(\bA, \bX)$. Since permuting node orders does not change a graph $G$, $p(\bA, \bX)$ needs to be permutation-invariant or an exchangeable distribution. Specifically, for an arbitrary node permutation $\pi: \{1, \ldots, N\} \rightarrow \{1, \ldots, N\}$, $p(\bA, \bX)$ needs to satisfy:
%\begin{align}
%    p(\bA,\bX) = p(\bA[\pi, \pi],\bX[\pi])
%    \label{eq:perm-invar} 
%\end{align}
%Here $\bA[\pi, \pi]$ represents permuting the first and second ranks of $\bA$ with $\pi$, and $\bX[\pi]$ represents permuting the rows of $\bX$ with $\pi$.}

% Denote $\calA(G)$ to be the set that contains all the pairs that lead to graph $G$, the log-likelihood $\log{p(G)}$ is defined as follow
% \begin{align}
%     \log{p(G)} = \log\sum_{(\bA,\bX)\in\calA(G)} p(\bA,\bX)
% \end{align}
% the form of joint distribution $p(\bA,\bX)$ can be categorized as inexchangeable distribution and exchangeable distribution. Early works [] formulate $p(\bA,\bX)$ using the former one as it is easier to design, and attempt to maximize a lower bound of $\log{p(G)}$ by choosing a heuristic subset of $\calA(G)$, such as BFS orderings. To obtain the exchangeable property, several works [] propose to use a permutation-invariant network to parameterize $p(\bA,\bX)$. As an exchangeable $p(\bA,\bX)$ equally assigns probability density to each $(\bA,\bX)$ in $\calA(G)$, the log-likelihood of $G$ can be written as
% \begin{align}
%     \log{p(G)}=\log{|\calA(G)|p(\bA,\bX)}
% \end{align}
% because the factor $|\calA(G)|$ is a constant [], one can directly maximize $p(\bA,\bX)$ without considering the node permutation. In this work, we model the distribution of graphs by maximizing the likelihood on an exchangeable distribution $p(\bA,\bX)$.

% \subsection{Score-based Generative Modeling}
% \red{Xiaohui: should we unify the notation of (L)SGM and our paper?}

% SGM diffusion
% v1
%{A score-based diffusion model defines a distribution with an approximate inverse of a  Gaussian diffusion process. Denote a Gaussian diffusion process by $(\bz_t: t \in [0, 1])$ and assume $\bz_0$ is from a base distribution $p_0(\bz_0)$. Assuming that the diffusion process is from an It\red{o} SDE []: 
% \begin{align}
%     \mbox{d}\bz = f(t)\bz \mbox{d}t + g(t) \mbox{d}\bw \label{sde}
% \end{align}
 %where $\bw$ is the standard Wiener process, and $f(t), g(t)$ are the scalar functions  respectively known as drift coefficient and diffusion coefficient, which are chosen so that the ending distribution of $\bz_1$ is a standard multivariate Gaussian distribution. An intuitive explanation of the diffusion process is to perturb the base distribution $p_0(\bz)$ with multiple noise scales, which are determined by time $t$, and finally obtain a standard Gaussian distribution $p_1(\bz)$ at $t=1$.}

Denote a continuous time diffusion process as $(\mathbf{Z}^t)_{t\in[0,1]}$ with base distribution $q_0(\mathbf{Z}^0)$. In practice, $q_0$ can either be the data distribution or latent variable distribution. Assuming the diffusion process follows an It\^{o} SDE:
\begin{align}
    \mbox{d}\bZ^t = f(t)\bZ^t \mbox{d}t + g(t) \mbox{d}\bW^t, \label{sde}
\end{align}
where $\bW^t$ is the standard Wiener process. $f(t)$ and $g(t)$ are scalar functions denoting drift and diffusion coefficients, which are chosen such that $q_1(\bZ^1)=\mathcal{N}(\bZ^1;\mathbf{0},\bI)$. The forward SDE gradually corrupt the base distribution to a random noise distribution that is easy to sample from, e.g., Gaussian distribution. To sample from the base distribution, we first draw $\bZ^1$ from $\mathcal{N}(\bZ^1;\mathbf{0},\bI)$ and run a reverse-time SDE:
\begin{align}
    \mbox{d}\bZ^t = [f(t)\bZ^t -g(t)^2\nabla_{\bZ^t}\log{q_t(\bZ^t)}]\mbox{d}t + g(t) \mbox{d}\bar{\bW}^t, \label{reverse-sde}
\end{align}
where $\bar{\bW}^t$ is the reverse-time standard Wiener process, and $q_t(\bZ^t)$ is the marginal distribution of the forward SDE at time $t$. Since $q_t(\bZ^t)$ is analytically intractable, we use a noise conditional score network $\epsilon_{\theta}(\bZ^t,t)$ to fit the score function as:
\begin{align}
    \min_\theta~~\mathbb{E}_{t\sim U[0,1]}\Big[\frac{g(t)^2}{2}\mathbb{E}_{q_0(\bZ^0)}\mathbb{E}_{q(\bZ^t|\bZ^0)}[\|\nabla_{\bZ^t}\log{q_t(\bZ^t)}-\epsilon_{\theta}(\bZ^t,t)\|^2_2]\Big],
\end{align}
where $q(\bZ^t|\bZ^0)$ denotes the transition kernel of forward SDE. Replacing $\nabla_{\bZ^t}\log{q_t(\bZ^t)}$ with the score network $\epsilon_{\theta}(\bZ^t,t)$ in Eqn.~(\ref{reverse-sde}) derives a score-based generative model (SGM). We denote the marginal distribution of SGM at $t=0$ as $p_\theta(\bZ)$.
% \red{Should we introduce $\epsilon$ in here? as it's used the NSCN part}
% v1
% An approximate reverse of the diffusion process defines $p_0(\bz_0)$, which is a flexible distribution and can be used for data fitting. A sample $\bz^0\sim p_0(\bz)$ can be obtained by first sampling $\bz^1$ from the base distribution $p_1(\bz)$ and then solving a reversed-time SDE:
% \begin{align}
%     \mbox{d}\bz = [f(t)\bz -g(t)^2\nabla_\bz\log{q_t(\bz)}]\mbox{d}t + g(t) \mbox{d}\bar{\bw} \label{reverse-sde}
% \end{align}
% where $\bar{\bw}$ is the standard Wiener process. The distribution $p_t(\bz_t)$  is the marginal distribution from the diffusion process. To fit the process, we often approximate $\nabla_\bz\log{q_t(\bz)}$ with a \textit{score network} $\bepsilon_\theta(\bz, t)$ parameterized by $\theta$. Estimating $\theta$ is the core of learning the diffusion process.}

%which is trained by minimizing the score matching objective []:
%\begin{align}
%    \theta^* = \underset{\theta}{\mathrm{argmin}}~\bbE_{t}\Big[\lambda(t)\bbE_{p_0(\bz^0)}\bbE_{q(\bz^t|\bz^0)}\big[||\nabla_{\bz^t}\log{q(\bz^t|\bz^0)} - \bepsilon_\theta(\bz^t, t)||^2_2\big]\Big] + C \label{score-matching}
%\end{align}
%where $t$ is uniformly sampled over $[0,1]$, $\lambda(t)$ is a weighting function of time $t$, $q(\bz^t|\bz^0)$ is a forward transition kernel which often comes with a closed-form. Here, $C$ is some constant irrelevant to the objective optimization w.r.t to parameter $\theta$ []. [] shows that when $\lambda(t)={g(t)^2/2}$, minimizing Eq. \eqref{score-matching} is equivalent to maximizing the lower bound of the data log-likelihood. 

% v1
% {While various methods directly fit data with $p_0(\bz_0)$, LSGM uses $p_0(\bz_0)$ as a flexible prior in a Variational Auto-Encoder (VAE). Let $\bx$ denote the observed random variable. Suppose the decoder and encoder of the VAE are $p_\psi(\bx | \bz_0)$ and  $q_\phi(\bz_0 | \bx)$ respectively, then the variational lower bound of the data log-likelihood $p(\bx)$ is:
% \begin{align}
%     \mathcal{L}(\bx; \theta, \psi, \phi) = \mathbb{E}_{q_\phi(\bz_0|\bx)}\big[\log{p_\psi(\bx|\bz_0)}\big] + \mathbb{H}\big[q_\psi(\bz_0|\bx)\big] - \mathbb{CE}\big[q_\psi(\bz_0|\bx)||p_\theta(\bz_0)\big]
    \label{eq:general-elbo}
% \end{align}
% Here the entropy term $\mathbb{H}\big[q_\psi(\bz_0|\bx)\big]$ is relative easy to calculate if $q_\psi$ takes a simple form. The cross entropy term needs some effort to calculate.  [] show that the cross entropy between the approximate posterior $q_\psi(\bz_0|\bx)$ and the SGM prior $p_\theta(\bz_0)$ is:
% \begin{align}
%     \mathbb{CE}\big(q(\bz^0|\bx)||p(\bz^0)\big)=\bbE_t\Big[\frac{g(t)^2}{2}\bbE_{q(\bz^0|\bx)}\bbE_{q(\bz^t|\bz^0)}\big[||\nabla_{\bz^t}\log{q(\bz^t|\bz^0)} - \bepsilon_\theta(\bz^t, t)||^2_2\big]\Big] +C \label{ce-mse}
% \end{align}
% By maximizing the lower bound in \eqref{eq:general-elbo}, we can learn model parameters $\theta$, $\psi$, and $\phi$.}

% In our graph generation problem, we need to define $p(\bx | \bz), q(\bz | \bx), epsilon(\bz, t)$. 
% where $C$ is a constant related to the approximate posterior and irrelevant to the objective optimization, and the score $\nabla_{\bz^t}\log{p(\bz^t)}$ is again estimated by a score network $\bepsilon_\theta(\bz^t, t)$ similar to Eq. \eqref{score-matching}.

% \subsection{Score-based Generative Modeling}
% % \red{Xiaohui: should we unify the notation of (L)SGM and our paper?}

% % SGM diffusion
% The score-based generative models [] are interested in modeling data distribution $p_0(\bz)$. Specifically, SGMs construct a diffusion process $\{\bz^t\}_{t=0}^{t=1}$, where $t\in[0,1]$ is a continuous time variable, so that $\bz^0=\bz$ is from the $p_0(\bz)$ and $\bz^1$ is from some base distribution $p_1(\bz)$ such as standard Normal. Here the diffusion process is modeled as the solution to an It\red{o} SDE []: 
% \begin{align}
%     \mbox{d}\bz = f(t)\bz \mbox{d}t + g(t) \mbox{d}\bw \label{sde}
% \end{align}
% where $\bw$ is the standard Wiener process, and $f(t), g(t)$ are the scalar functions known as drift coefficient and diffusion coefficient, respectively. The intuitive explanation of the diffusion process is to perturb the data distribution $p_0(\bz)$ with multiple noise scales, which are determined by time $t$, and finally obtain a base distribution $p_1(\bz)$ at $t=1$. 

% % SGM reverse-diffusion (denoising)
% A sample $\bz^0\sim p_0(\bz)$ can be obtained by first sampling $\bz^1$ from the base distribution $p_1(\bz)$ and then solving a reversed-time SDE:
% \begin{align}
%     \mbox{d}\bz = [f(t)\bz -g(t)^2\nabla_\bz\log{q_t(\bz)}]\mbox{d}t + g(t) \mbox{d}\bar{\bw} \label{reverse-sde}
% \end{align}
% where $\bar{\bw}$ is the standard Wiener process. The score of the distribution $\nabla_\bz\log{q_t(\bz)}$ can be estimated using a score network $\bepsilon_\theta(\bz, t)$ parameterized by $\theta$, which is trained by minimizing the score matching objective []:
% \begin{align}
%     \theta^* = \underset{\theta}{\mathrm{argmin}}~\bbE_{t}\Big[\lambda(t)\bbE_{p_0(\bz^0)}\bbE_{q(\bz^t|\bz^0)}\big[||\nabla_{\bz^t}\log{q(\bz^t|\bz^0)} - \bepsilon_\theta(\bz^t, t)||^2_2\big]\Big] + C \label{score-matching}
% \end{align}
% where $t$ is uniformly sampled over $[0,1]$, $\lambda(t)$ is a weighting function of time $t$, $q(\bz^t|\bz^0)$ is a transition kernel which often comes with a closed-form. Here, $C$ is some constant irrelevant to the objective optimization w.r.t to parameter $\theta$ []. [] shows that when $\lambda(t)={g(t)^2/2}$, minimizing Eq. \eqref{score-matching} is equivalent to maximizing the lower bound of the data log-likelihood. 

% % LSGM
% Relying on the variational auto-encoder (VAE) framework, [] proposes to train a SGM in the latent space. Specifically, [] uses SGM to model the flexible prior $p(\bz)$ and show that the cross entropy between the approximate posterior $q(\bz^0|\bx)$ and the SGM prior $p(\bz^0)$ is:
% \begin{align}
%     \mathbb{CE}(q(\bz^0|\bx)||p(\bz^0))=\bbE_t\Big[\frac{g(t)^2}{2}\bbE_{q(\bz^0|\bx)}\bbE_{q(\bz^t|\bz^0)}\big[||\nabla_{\bz^t}\log{q(\bz^t|\bz^0)} - \bepsilon_\theta(\bz^t, t)||^2_2\big]\Big] +C \label{ce-mse}
% \end{align}

% In our graph generation problem, we need to define $p(\bx | \bz), q(\bz | \bx), epsilon(\bz, t)$. 


==> NIPS/sections/related_works.tex <==
\vspace{-1em}
\section{Related Works} \label{sec:related}
\textbf{Score-based generative models.} Score-based generative models~\citep{song2019generative,ho2020denoising,song2020score} have shown effective at the generation of data in various domains \citep{ho2020denoising,chen2020wavegrad,niu2020permutation}. In SGMs, data are first diffused with gradually increasing noise, and the model learns to estimate the score at each noise scale. During generation, an SGM first randomly draws some noise from a simple distribution and then decreases the noise scales sequentially to obtain a sample. Instead of generating data directly, \citet{mittal2021symbolic,sinha2021d2c,wehenkel2021diffusion,vahdat2021score} utilize SGM in latent space and turn it into a flexible prior by combining the VAE framework~\citep{kingma2013auto}. \scriptupdate{Unlike approaches that use more complex prior \citep{dai2019diagnosing,klushyn2019learning}, SGM prior addresses the posterior mismatch problem by construction \citep{sinha2021d2c}. Combining SGM prior into VAE framework also enables faster sampling as well as hierarchically generating data.}

\textbf{Graph generation models.} Current graph generative models sample graphs either autoregressively or in one-shot. 
%Auto
Autoregressive graph generative models generate graphs by adding nodes and edges sequentially~\citep{you2018graphrnn,li2018multi,li2018learning,jin2018junction,liao2019efficient,shi2020graphaf,zang2020moflow,bacciu2020edge,dai2020scalable,goyal2020graphgen,tran2020deepnc,luo2021graphdf, bengio2021flow}. 
Training such models requires a particular node ordering from the graph to pin down the generation sequence, thus unable to preserve the model exchangeability~\citep{chen2021order}. Besides, the autoregressive models usually fail to learn the global structure of a graph as they can not capture the long-term dependency. 
%oneshot
The other type of models generate graph in one-shot~\citep{simonovsky2018graphvae,liu2018constrained,madhawa2019graphnvp,kajino2019molecular,bradshaw2019model,grover2019graphite,lim2020scaffold,jin2020hierarchical,guo2020node,lippe2020categorical,samanta2020nevae,niu2020permutation,garcia2021n,jo2022score}. Unlike autoregressive models, exchangeability can be preserved through carefully designing the model architecture. However, those models need to generate nodes and edges in parallel and can not scale up to large graphs. 
%vgae   
On par with the one-shot graph generative models, VGAEs~\citep{kipf2016variational,mehta2019stochastic,liu2019graph,li2020dirichlet} adopt the variational inference framework to learning node representations that are useful for downstream tasks, such as unsupervised learning or node clustering. However, The merits of using such approaches in graph generation, such as the exchangeable property and the parallel sampling scheme, have not been fully exploited. 
%our work
Our work builds on the VGAE framework and utilizes a learnable prior based on SGM.





==> NIPS/tables/chemical-main.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Performance on molecule generation. Extended NSPDK, Uniqueness and Novelty metrics as well as the standard deviations of all metrics are in Appendix \ref{app:extra-exp}.}
    \begin{tabular}{lcccccc}\hline
         &  \multicolumn{3}{c}{QM9} & \multicolumn{3}{c}{ZINC250K}\\
         &  Validity$\uparrow$ & FCD$\downarrow$ & Time (s)$\downarrow$ &Validity$\uparrow$ & FCD$\downarrow$  & Time (s)$\downarrow$ \\\hline
         GraphDF & 82.67 & 10.816 &5.35e4 & 89.03& 34.202 & 6.03e4\\
         MoFlow & 91.36 & 4.467 & \textbf{4.60} &63.11 & 20.931 &\textbf{24.5}\\
         GraphCNF &95.00&1.629&59.48&95.26&14.786&1.04e2\\
         EDP-GNN & 47.52  & 2.680 &4.40e3 & 82.97 & 16.737 & 9.09e3\\
         GDSS & 95.72 & 2.900 &1.14e2&\textbf{97.01} & 14.656 & 2.02e3 \\\hline
         NVDiff & \textbf{95.79} & \textbf{1.131} &10.71 &85.63&\textbf{4.019} &90.2\\\hline
        %  NVDiff-E & \textbf{98.49}& \textbf{0.350} &  15.64&\textbf{96.23}&6.681&2.01e2\\
    \end{tabular}
\vspace{-15pt}
    \label{tab:molecule}
\end{table}
% \begin{table}[t]
%     \centering
%     \small
%     \caption{Performance on molecule generation. ``-'' indicates results not available. Extended NSPDK, Uniqueness and Novelty metrics as well as the standard deviations of all metrics are in \red{Appendix}.}
%     \begin{tabular}{lcccccccc}\hline
%          &  \multicolumn{4}{c}{QM9} & \multicolumn{4}{c}{ZINC250K}\\
%          &  Validity$\uparrow$ & FCD$\downarrow$ & NLL$\downarrow$ & Time (s)$\downarrow$ &Validity$\uparrow$ & FCD$\downarrow$ & NLL$\downarrow$ & Time (s)$\downarrow$ \\\hline
%          GraphDF & 82.67 & 10.816 &-&5.35e4 & 89.03& 34.202 &-& 6.03e4\\
%          MoFlow & 91.36 & 4.467 &-& \textbf{4.60} &63.11 & 20.931 &-&\textbf{24.5}\\
%          EDP-GNN & 47.52  & 2.680 &-&4.40e3 & 82.97 & 16.737 &-& 9.09e3\\
%          GraphCNF &95.00&1.629&27.66&59.48&95.26&14.786&\textbf{84.25}&1.04e2\\
%          GDSS & 95.72 & 2.900 &-&1.14e2&\textbf{97.01} & 14.656 &-& 2.02e3 \\\hline
%          NVDiff & 95.79 & 1.131 &\textbf{25.61}&10.71 &85.63&\textbf{4.019} &93.41&90.2\\
%          NVDiff-E & \textbf{98.49}& \textbf{0.350} &42.50&  15.64&\textbf{96.23}&6.681&87.78&2.01e2\\\hline
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[]
%     \centering
%     \small
%     \begin{tabular}{lcccccccccc}
%          &  \multicolumn{5}{c}{QM9} & \multicolumn{5}{c}{ZINC250K}\\
%          &  Validity & NSPDK & FCD & NLL & Time (s) & Validity & NSPDK & FCD & NLL&Time (s) \\\hline
%          GraphDF & 82.67 & 0.063 & 10.816 &-&5.35e4 & 89.03 & 0.176 & 34.202 &-& 6.03e4\\
%          MoFlow & 91.36 &0.017 & 4.467 &-& 4.60 &63.11  & 0.046 & 20.931 &-&24.5\\
%          EDP-GNN & 47.52 & 0.005 & 2.680 &-&4.40e3 & 82.97 & 0.049 & 16.737 &-& 9.09e3\\
%          GraphCNF &95.00&0.002&1.629&27.66&59.48&95.26&0.046&14.786&84.25&1.04e2\\
%          GDSS & 95.72 & 0.003 & 2.900 &-&1.14e2&97.01 & 0.019 & 14.656 &-& 2.02e3 \\\hline
%          NVDiff & 95.79 & 0.002& 1.131 &25.61&10.71 &85.63&0.066&4.019 &93.41&90.2\\
%          NVDiff-E & 98.49&  0.002 & 0.350 &&  15.64&96.23&0.061&6.681&&2.01e2\\\hline
%     \end{tabular}
%     \caption{Main table}
%     \label{tab:my_label}
% \end{table}

==> NIPS/tables/common-main.tex <==

\begin{table}[h]
\vspace{-1em}
    \centering
    \small
    % \floatbox[\capbeside]{table}
    % {\caption{A test table with its caption beside}}
    % \caption{Performance on generic graph generation. ``-'' indicates results not available and ``OOM'' indicates Out of Memory.}
    \caption{Performance on generic graph generation. ``OOM'' denotes out of memory.}
    \begin{tabular}{lcccccccc}\hline
    &\multicolumn{4}{c}{Community-small} & \multicolumn{4}{c}{Ego-small}\\
    &Deg.$\downarrow$ & Clus.$\downarrow$ &Orbit$\downarrow$ &\scriptupdate{NN$\downarrow$} & Deg.$\downarrow$& Clus.$\downarrow$ &Orbit$\downarrow$&\scriptupdate{NN$\downarrow$}\\\hline
    GraphRNN & 0.080 & 0.120 & 0.040 &\scriptupdate{0.997}& 0.090 & 0.220 & 0.003 &\scriptupdate{\textbf{1.094}}\\
    GRAN& 0.070 & 0.045 & 0.021 &\scriptupdate{0.701}& 0.020&0.126&0.010 &\scriptupdate{\textbf{1.095}}\\
    GraphCNF & \textbf{0.021} & 0.141 & 0.044 &\scriptupdate{0.876}& 0.011 & \textbf{0.011} & \textbf{0.001} &\scriptupdate{\textbf{1.094}}\\
    EDP-GNN & 0.053 & 0.144 & 0.026 &\scriptupdate{0.789}& 0.052 & 0.093 & 0.007&\scriptupdate{\textbf{1.095}}\\
    GDSS &  0.045 & 0.086 & \textbf{0.007} &\scriptupdate{0.858}& 0.021 & 0.024 & 0.007 &\scriptupdate{1.097}\\\hline
    NVDiff & \textbf{0.021} & \textbf{0.035} & 0.018 &\scriptupdate{\textbf{0.688}}& \textbf{0.005} & 0.045 & \textbf{0.001} &\scriptupdate{\textbf{1.092}}\\\hline
    &\multicolumn{4}{c}{Community} & \multicolumn{4}{c}{Ego}\\
    &Deg.$\downarrow$ & Clus.$\downarrow$ &Orbit$\downarrow$ &\scriptupdate{NN$\downarrow$} & Deg.$\downarrow$& Clus.$\downarrow$ &Orbit$\downarrow$&\scriptupdate{NN$\downarrow$}\\\hline
    GraphRNN & \textbf{0.014} &\textbf{0.002}& 0.039 &\scriptupdate{1.452}& 0.077 &0.316& 0.030 &\scriptupdate{0.192}\\
    GRAN &  0.085 & 0.068 &0.042 &\scriptupdate{1.406}& 0.064 & 0.279 & 0.039 &\scriptupdate{0.196}\\
    GraphCNF & 0.707 & 1.305 & 0.194 &\scriptupdate{1.356}& OOM&OOM&OOM &\scriptupdate{OOM}\\
    EDP-GNN & 0.137 &1.104 & 0.051 &\scriptupdate{1.146}& 0.069&0.447&0.055 &\scriptupdate{\textbf{0.189}}\\
    \scriptupdate{GDSS} & \scriptupdate{0.099} & \scriptupdate{0.327} & \scriptupdate{0.162} &\scriptupdate{1.203}&\scriptupdate{0.134} & \scriptupdate{0.372} & \scriptupdate{0.139} &\scriptupdate{0.295}\\\hline
    NVDiff &0.093&0.086&\textbf{0.021}&\scriptupdate{\textbf{0.982}}& \textbf{0.045}& \textbf{0.091}&  \textbf{0.004} &\scriptupdate{0.195}\\\hline
    \end{tabular}
    \vspace{-0.35cm}
    \label{tab:generic}
\end{table}
% \begin{table}
%     \centering
%     \small
%     % \small 67.02 citeseer: 55.53
%     % \captionsetup{singlelinecheck = false, format= hang, justification=raggedright, font=footnotesize, labelsep=space}
%     \caption{Performance on generic graph generation. ``-'' indicates results not available and ``OOM'' indicates Out of Memory.}
%     \begin{tabular}{lcccccccc}\hline
%     &\multicolumn{4}{c}{Community-small} & \multicolumn{4}{c}{Ego-small}\\
%     &Deg.$\downarrow$ & Clus.$\downarrow$ &Orbit$\downarrow$ & NLL$\downarrow$ & Deg.$\downarrow$& Clus.$\downarrow$ &Orbit$\downarrow$ & NLL$\downarrow$\\\hline
%     GraphRNN & 0.080 & 0.120 & 0.040 &-& 0.090 & 0.220 & 0.003&-\\
%     GRAN& 0.070 & 0.045 & 0.021 &- &0.020&0.126&0.010 &-\\
%     % GraphDF & 0.060 & 0.120 & 0.030 &-& 0.040 & 0.130 & 0.010&-\\
%     % GraphNF & 0.120 & 0.150 & 0.020 &-& 0.030 & 0.100 & \textbf{0.001}&-\\
%     GraphCNF & \textbf{0.021} & 0.141 & 0.044 &67.02& 0.011 & \textbf{0.011} & \textbf{0.001} & \textbf{55.53}\\
%     EDP-GNN & 0.053 & 0.144 & 0.026 &-& 0.052 &  0.093 & 0.007&-\\
%     GDSS &  0.045 & 0.086 & \textbf{0.007} &-& 0.021 & 0.024 & 0.007 & -\\\hline
%     NVDiff & \textbf{0.021} & \textbf{0.035} & 0.018 & \textbf{47.89}& \textbf{0.005} & 0.045 & \textbf{0.001} & 56.23\\\hline
%     % NVDiff & \textbf{0.021} & \textbf{0.035} & 0.018 & 2.3s(time)& \textbf{0.005} & 0.045 & \textbf{0.001} & 2.6s(time)\\
%     &\multicolumn{4}{c}{Community} & \multicolumn{4}{c}{Ego}\\
%     &Deg.$\downarrow$ & Clus.$\downarrow$ &Orbit$\downarrow$ & NLL$\downarrow$ & Deg.$\downarrow$& Clus.$\downarrow$ &Orbit$\downarrow$ & NLL$\downarrow$\\\hline
%     GraphRNN & \textbf{0.014} &\textbf{0.002}& 0.039&-&0.077 &0.316& 0.030&-\\
%     GRAN &  0.085 & 0.068 &0.042 &-& 0.064 & 0.279 & 0.039&-\\
%     GraphCNF & 0.707 & 1.305 & 0.194 & \textbf{4138}&OOM&OOM&OOM&OOM\\
%     EDP-GNN & 0.137 &1.104 & 0.051&-&0.069&0.447&0.055&-\\\hline
%     NVDiff &0.093&0.086&\textbf{0.021}&4831& \textbf{0.045}& \textbf{0.091}&  \textbf{0.004}&3602\\\hline
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}


==> aaaireview.tex <==
We thank all reviewers for their valuable feedback. We want to summarize our contributions again here.

This work aims to reduce the dimension of diffusion processes for graph generation tasks. We achieve this goal by diffusing node vectors only. This method does use the known VGAE framework, but it would not work without our two innovations in model architectures.
- score network: we enhance node vectors' ability to encode graph structures by introducing an extra global context vector. 
- decoder: we introduce a GNN to recover a graph from node vectors only (note that there are only node vectors but not a graph for message-passing. Previous models (e.g., VGAE) directly recover an edge from two node vectors).

Below we address questions from each reviewer.


--R3--

Q1. ablation study.
A1. We provide ablation studies of the context vector and the regularization term in the appendix. We have also explored other design choices in the development of our method. For example, we have tried the encoder and decoder of VGAE but did not find they work. Attention-based scoring is a natural choice since we have a set of vectors as the input. Previous diffusion-based generative models have the graph structure and use GNNs, but we don't have the graph structure and cannot make such a comparison.


--R5--

Q1. "the paper adds little to the knowledge of the community"
A1. The knowledge from this work is that good-quality graphs can be generated from node vectors only. We don't see this finding in the literature prior to our work. VGAE is not designed for graph generation because its purpose is "learning interpretable representations" [Kipf and Welling 2016]. We greatly reduce the latent dimension of diffusion processes, which is not explored by previous diffusion-based graph generative models.  

Q2. "without a clear discussion of what are the key methodological differences" 
A2. As we mentioned in the abstract, the key innovation is to reduce the dimension of diffusion processes by modeling node vectors only. We directly compare our model against two previous diffusion-based methods, EDP-GNN and GDSS, and show the improvement in efficiency and quality of generation.

Q3. The novelty metric.
A3. Note that QM9 enumerates all molecules with less than nine heavy atoms in the chemical space [1]. It can be considered the entire distribution. Thus, a well-fitted model will likely have low novelty scores (generated molecules appear in the training set). This issue is also discussed by [2]. Here we did a little investigation, which somewhat deviates from our main point, so we put it in the appendix. 

[1] Ruddigkeit et al. Enumeration of 166 billion organic small molecules in the chemical universe database gdb-17. JCIM 2012.
[2] Vignac. et al. Top-N: Equivariant set and graph generation without exchangeability. ICLR 2022.

Q4. Validity & efficiency.
A4. There are three reasons that our model is preferred. 
- The proposed model is for general graph generations, many of which do not have a validity metric.
- We argue that metrics like FCD are more important because they measure generated molecules' usefulness. 
- On ZINC, our model is lower than GDSS by 12% in validity but faster by 2200% in speed. Our model still generates valid molecules much faster than the SOTA baseline.  

Q5. GNN on fully connected graphs.
A5. We politely argue that a GNN on fully connected graphs does not amount to an MLP. GNN is an equivariant function on graphs, while an MLP is not in general.

Q6. Ablation study of graph encoding.
A6. We include the graph encoder in section 3.5 for completeness but don't consider it our innovation. Using extra edges and noise injection are both techniques from the literature. 


Q7. "novelties ... when compared to the single most related works in literature?"
A7. The most relevant model is GDSS, compared with which our model has the major advantage of reducing the diffusion dimension. We further make two innovations (3.3 and 3.4) to devise a model within the VGAE framework.   

--R6--

Q1. The proposed technique seems to be directly adapted from the diffusion model. 
A1. We hope the general response address the reviewer's concerns.

Q2. graph decoding and encoding "are not novel." 
A2. Our decoding method is new. We have several considerations in this design. For example, edge vectors are computed as differences between node vectors. 
Compared to methods (e.g., GraphNF) that compute edge weights for an adjacency matrix, our method takes an easier form to restore edge information. 

Q3. SOTA baselines.
A3. We believe GDSS is the SOTA work. A comparison against it should support the findings of this work.

--R7--

Q1. Sampling steps & hardware requirements.
A1. We report average sampling steps here -- QM9(53), ZINC(195), Com.-small(25), Com.(32), Ego-small(35), Ego(51). We experiment on RTX 3060/6000 and A100 GPUs. For sampling speed, all results are obtained with 5 different random seeds using RTX 3060.






% R3.
% Q1. "ablation study"
% A1. We agree that many components are proposed. We provide the ablation study of the context vector and the regularization term in the appendix. For the VGAE, We also explore other design choices for the encoder and decoder when developing our method and will include those results in the manuscript. However, for other components, we explore less as the SGM prior and the attention-based scoring work effectively at the beginning. We believe other more reasonable designs can further improve the performance and would to leave them to future work.

% R5.
% Q1. "the paper adds little to the knowledge of the community"

% A1. The knowledge from this work is that good-quality graphs can be generated from node vectors only. We don't see this finding in the literature before our work. Note that VGAE is not designed for graph generation because its purpose is "learning representations". Upon this finding, we greatly reduce the latent dimension of diffusion processes, which is also not explored by previous diffusion-based graph generative models.  

% Q2. "Clear and direct comparison between the proposed model and those in literature" 

% A2. Since we want to show the benefit of reducing the dimension of diffusion processes in graph generation, we directly compare our model to two diffusion-based methods, EDP-GNN and GDSS. The results show that our model is much faster than EDP-GNN and GDSS. Furthermore, our model can generate high-quality molecules in various tasks. 



% Q3. Issues with the novelty metric

% A3. We'd like to point out that QM9 is special -- it enumerates all molecules with less than 9 heavy atoms in the chemical space [1]. It can be considered the entire distribution. Therefore, it is very likely that a model fitting the data well has low novelty values (generated molecules appear in the training set). 

% This issue is also discussed by [2]. Here we did a little investigation in the appendix. We believe this investigation deviates from our main point, so we put it in the appendix. 

% [1] Ruddigkeit et al. Enumeration of 166 billion organic small molecules in the chemical universe database gdb-17. Journal of chemical information and modeling 2012.

% [2] Vignac. et al. Top-N: Equivariant set and graph generation without exchangeability. ICLR 2022.

% Q4. Validity and efficiency

% A4. There are several reasons that our model is preferred. First, the proposed model is for general graph generations, many of which do not have a validity metric. Second, validity is just one metric in molecule generation, and we argue that other metrics like FCD scores are more important because it measures the usefulness of generated molecules. 
% Third, the validity of our model is lower than GDSS by 12% but faster than it by 2200%, our model still can generate valid molecules much faster than the sota baseline.  

% Q5. Reason for using GNN on fully connected graphs

% A5. We politely argue that a GNN on fully connected graphs does not amount to an MLP. GNN is an equivariant function on the graph while an MLP is not in general. Existing literature [1,2] frequently apply GNNs on fully connected graphs.

% [1] Satorras et al. E (n) equivariant graph neural networks. ICML 2021.

% [2] Köhler et al. Equivariant flows: sampling configurations for multi-body systems with symmetric energies. ICML 2020.

% Q6. "Ablation study of graph encoding"

% A6. Due to the time limit of the rebuttal period, we'd like to provide you with the reconstruction quality on ZINC datasets for graph encoding with and without the extra edge type. Specifically, we can recover 98% of edges with extra edge type and 65% when without. The result will be updated in the next version.

% Q7. "methodological novelties"

% A7. The most relevant model is GDSS. Compared with GDSS, our model has the major advantage of reducing the diffusion dimension. 
% In particular, modeling node vectors only in the VGAE framework is already a step forward. Furthermore, we innovate two techniques to make the model work better. 

% - Score network: we introduce the global context vector to attend each node vector, which is very useful in terms of guiding the generation direction of a graph.

% - Decoder: we innovate the GNN to decode node and edge types from node vectors.

% We sincerely hope this addresses the reviewer's concerns about our novelties. [general response to all reviewers?]


% R6

% -1&2- "The proposed technique seems to be directly adapted from the diffusion model"
% Thanks to the reviewer's comment, we realized that the contribution of this paper was not sufficiently clear. The original diffusion-based generative models have demonstrated effective in generating 2D images. However, there are significant differences between the image data and the graph: the graph is discrete, unordered and irregular. These differences make it non-trivial to utilize the diffusion model on graphs.
% "Both graph decoding and encoding are straightforward and subtle technical design is desired."
% Refer to the A7.


% Q2. “sota baselines”
% A2. The baselines are sota during the development of our work. We will add newer baselines to the experiments in the next version. (need revised)

% R7
% We thank the reviewer for the feedback! We will fix the mentioned typo.

% Q1. Detail of sampling and hardware requirements.
% A1. The required sampling steps depend on the complexity of the graphs, we show the average sampling steps for each dataset -- QM9(53), ZINC(195), community-small(25), community(32), Ego-small(35), Ego(51).  We run experiments on GeForce RTX 3060/6000, and A100 GPUs. For sampling speed, all results are obtained by 5 runs with different random seeds using RTX 3060.



Message to SPC.

Dear SPC: 

We'd like to point out a factual misunderstanding in Question 1 of R5. R5 thinks that a GNN on a complete graph "will basically amount to use a simple MLP taking in input information from all nodes in the graph (with appropriate weight sharing)". But we believe this point is wrong because GNN is an equivariant function (a permutation of the input gives an output with the same permutation), but an MLP is not equivariant in general. We hope this misunderstanding does not factor into the evaluation of our submission. 

Thank you!

==> nipsreview.tex <==
##Reviewer 1 
Summary:
The paper tackles the problem of graph generation using a VGAE architecture combined with a score-based generative model (SGM) as a flexible prior to sample node vectors. The generative process first samples a latent representation of the graph as node vectors Z (O(N)) before decoding graph adjacency and node features conditioning on the latent representation, using a GNN as core component. NVDiff is trained end-to-end by optimizing the variational lower bound of log-likelihood. Various experiments are designed to evaluate several aspects of the graph generation process.

Strengths And Weaknesses:
Strengths:
1. The paper is well-written and easy to follow. Concepts are well defined, notation is sound, figures are informative.
2. The work is well related to baselines. Enough background is provided.
3. The proposed idea is clear and relevant. The contribution seems decent to me: use SGM prior with specific attention-based scheme in VGAE architecture (node exchangeability follows), model only node vectors in latent space (scalability follows), some architectural designs.
4. Diverse experiments are presented. Results are favorable.
Weaknesses:
1. The main limitation to me is the total absence of ablation study. Without it, it seems impossible to judge the real benefits of some additions brought by the paper. We can only judge the framework as a whole. For instance, is the global_vector_0 beneficial? Does using a GNN in the encoder help? What about the consistency regularization term? Is considering non-edges as an extra type worth it given the extra cost in complexity induced? Although I understand that not everything can be tested, showing the benefits of some main contributions of the paper seems essential to me.

Minor points / Suggestions:
1. "Flow network based generative models for non-iterative diverse candidate generation, Bengio et al., NeurIPS 2021. as a reference for normalizing flow approaches.
2. State where the metrics in 5.1, line 240 are reported. (Table 6 of Appendix I believe).
3. At the start of the Experiments section, introduce clearly the different aspects that are being investigated. (e.g. generation performance on real-world datasets, speed, contextual vector information, visualisation, community patterns of node vectors, etc.). This will make it clearer for the reader.
4. Motivate more clearly all benefits of using SGM prior instead of Gaussian prior in VGAE.
5. The Z_i^t in the score network (Section 3.3, line 125) could be described more rigorously than "a corrupted sample from the encoder".
 
Questions:
1. Could you describe a bit more why using the adjacency matrix E constructed from Z makes sense in the decoder part? I understand what it represents but what makes it a good choice to learn A,X using the proposed GNN? No intuition is provided while this is a key component to enable deriving only node vectors in the latent space, a core contribution of the paper.
2. On a similar note, this adjacency E forms a complete graph. The applied GNN (eq. (9)) will thus show high complexity (O(N^2)). Can you discuss the scalability? In different terms, you do not consider edges in the latent space, but still consider them in the rest of the network. What is the expressivity / scalability trade-off here?
3. Can you justify why GNN considers non-edges type in Eq. (14)?
4. Especially for the performance of molecule generation (table 1), can we see information about the loss optimization? Is there a component of the framework (e.g. reconstruction loss, cross-entropy loss, entropy term) that works best? More generally, could you elaborate a bit more (clearly) on the performance of each component of the framework?

Limitations:
Some limitations are evoked but this is succinct. Molecular generation can have a broad impact on the medical field, both positive and negative. The authors could elaborate on that.

Ethics Flag: No
Soundness: 3 good
Presentation: 3 good
Contribution: 3 good
Rating: 6: Weak Accept: Technically solid, moderate-to-high impact paper, with no major concerns with respect to evaluation, resources, reproducibility, ethical considerations.
Confidence: 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.
Code Of Conduct: Yes


##Author
Thank you for your feedback! We sincerely appreciate your feedback on our work. Please check our answers to your questions below.

Q1. the total absence of ablation study

Response: We have conducted two ablation studies about contextual embedding and consistency regularization. The first table below shows results with and without the contextual embedding vector . The study demonstrates that contextual embedding improves the validity and FCD metrics.

QM9		ZINC250K	
Validity	FCD	Validity	FCD
w/o cont. emb.	93.18	3.082	83.11	6.100
w/ cont. emb.	95.79	1.131	85.63	4.019
The second table shows the results with and without consistency regularization. The consistency regularization term improves validity scores, especially on the ZINC250K dataset.

QM9		ZINC250K	
Validity	FCD	Validity	FCD
w/o cons. reg.	94.24	1.021	71.35	4.295
w/ cons. reg.	95.79	1.131	85.63	4.019
Note that our model must need an encoder to map a graph to latent node vectors. A GNN is a natural choice for the encoder.

We will add the results above to our submission.

Q2. why using the adjacency matrix  constructed from  makes sense in the decoder part?

Response: We prefer to call  a “distance tensor” rather than an “adjacency tensor” since each entry  represents the squared difference for each pair of latent node vectors (, ) along each dimension . Thus,  can be explained as “coordinates” of node  in the latent space.

In contrast to approaches in [2,3], which compute distances between nodes, we do not aggregate differences across dimensions to keep more information for the decoder. We will add such a discussion to our submission.

Q3. scalability and expressivity of using full E matrices in the decoder.

Response: The computation of the decoder only takes a small fraction of the overall computation time because the diffusion process takes much more time, so the computation using a full E matrix does not significantly increase the running time. Compared with EDP-GNN and GDSS, our method mainly reduces the computation time of the diffusion process.

Our model may lose some expressivity by using fewer vectors, but it may gain back some expressivity because our latent space has a much lower dimensionality and is easier to model. The benefit of using a low-dimensional latent space is particularly clear on datasets with large graphs.

Q4. why GNN considers non-edges type in the encoder in Eq. (14).

Response: Non-edges add many more connections to the graph and accelerate message passing in a GNN layer. This method is already used in previous studies [1,2]. We also find this setting performs well in our model.

We agree that using non-edges increases encoder computation. But encoder is not the computational bottleneck in our model. In particular, we do not use the encoder during generation.

Q5. information about the loss optimization.

Response: We include the reconstruction loss of the VAE and the MSE loss in the table below. Note that the entropy term is a constant, and the MSE loss is an estimation of the cross-entropy term (differ by a constant). These numbers are from the optimization of the two terms on the QM9 dataset. We observe that the reconstruction loss converges faster than the MSE loss. This justifies why we optimize the parameters of the VAE and the diffusion prior separately so that the learning rates for the two sets of parameters can be different.

In our observation, the model cannot generate good samples before the MSE loss converges. We hypothesize that the prior is still too far from the posterior, and latent vectors from the diffusion process cannot be decoded into good graph samples (e.g. valid molecules).

If possible, can you be more specific about "the performance of each component of the framework"? Do you mean the optimization performance?

Epochs	100	200	300	400	500	600	700	800	900	1000
MSE loss (1e2)	8.781	7.676	7.571	7.51	7.481	7.471	7.442	7.425	7.422	7.418
Recon. loss (1e1)	13.16	5.184	4.632	4.409	4.299	4.24	4.416	4.144	4.208	4.205
References:

[1] Lippe et al. (2020). Categorical normalizing flows via continuous transformations. arXiv preprint arXiv:2006.09790.

[2] Satorras et al. "E (n) equivariant graph neural networks." International conference on machine learning. PMLR, 2021.

[3] Köhler et al. (2019). Equivariant flows: sampling configurations for multi-body systems with symmetric energies. arXiv preprint arXiv:1910.00753.

-------------------------------------------------------------------
##Reviewer 2
Summary:
This paper targets to design a graph generation model by integrating Variational Graph Auto-Encoder (VGAE) and SDE-based generative model. The proposed model is based on the framework of VGAE. The key modification is the Gaussian prior in VGAE is replaced by a score network, which is proposed in an SDE-based generative model (a Latent Score-based Generative Model (LSGM) from a NeurIPS’21 paper). In fact, this LSGM model itself leverages a variational autoencoder (VAE) framework and is a new approach for learning score-based generative models in latent space. In other words, this paper extends the application of LSGM in graph generation. The figure 1 of this paper and the figure 1 in LSGM paper show the same model framework.

Strengths And Weaknesses:
Strength: 
1) The paper is clearly written.
2) The model is evaluated on different types of graph generation.
Weakness 
1) The proposed method is highly similar to the LSGM model. The paper contributes more as an application of LSGM on graph generation. 
2) The molecular graph generation also uses important metrics such as uniqueness and novelty. The results in the appendix show that the proposed model has much lower novelty than baselines, and lower uniqueness on the QM9 dataset.

Questions:
The paper reports sampling speed in evaluation. How about the training cost?

Limitations:
NA

Ethics Flag: No
Soundness: 2 fair
Presentation: 3 good
Contribution: 2 fair
Rating: 3: Reject: For instance, a paper with technical flaws, weak evaluation, inadequate reproducibility and incompletely addressed ethical considerations.
Confidence: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
Code Of Conduct: Yes


##Author
Thank you for your feedback! We really appreciate your feedback! Below we answer your questions separately.

Q1. The proposed method is highly similar to the LSGM model. The paper contributes more as an application of LSGM on graph generation.

Response: We agree that our model is based on the LSGM, but we politely disagree that our method is a simple application of LSGM on graph generation tasks. In our view, LSGM cannot be directly applied to graph data. In particular, LSGM cannot address the permutation-invariant issue. The architectures of an existing LSGM are not designed to model graph structures either (e.g. capturing node relations). Modeling graphs requires advanced models such as EDP-GNN and GDSS.

We achieve permutation invariance in the latent space and make two innovations to achieve good performance in graph generation tasks.

First, we propose to use node vectors only in the latent space. Different from EDP-GNN and GDSS, we can use a much lower latent space, which not only brings computational efficiency but also makes it easier to model the latent distribution.

Second, we have designed a network architecture to achieve good generation performances. In particular, our design of the contextual vector has shown to be useful in graph generation tasks.

The contribution of our work is verified through experiments in the submission and also the ablation study in the reply to Reviewer Xkda. Overall, we think our model is one solid step forward for diffusion-based graph generation models.

Q2. the proposed model has much lower novelty than baselines, and lower uniqueness on the QM9 dataset.

Response: We would like to point out that the QM9 dataset is special here. It enumerates all organic small molecules with less than 9 heavy atoms in the chemical space [1, 2, 3] and thus can be considered as the entire distribution. Therefore, it is very likely that a good model fits the data well but has low novelty values (generated molecules appear in the training set (90% of the entire dataset)). Previous work such as [3] does not even include the evaluation of "novelty" for this dataset. We include this value for completeness.

We further train our model in 10% of the data, and the novelty value becomes 99.99%, which indicates that our model does not just memorize the training data.

There is a similar issue with "uniqueness" metric. Compared with a model with a large dispersion, our model concentrates more of its probability on the data and thus has slightly lower uniqueness values. It does not necessarily indicate that our model has worse data fitting than competing models.

Q3. How about the training cost?

Response: We compare the per-epoch training time of our model against GDSS on two datasets and report the per-epoch training time (in minutes) below. Note that the training procedure requires a model to run only a single denoising step. Our running time is comparable to GDSS. During generation, our model needs a much less number of denoising steps than GDSS (e.g. 70 vs 1000), so our model has a much faster speed.

QM9	ZINC250K
GDSS	4.16	6.89
NVDiff	3.5	8.64
References:

[1] Lars Ruddigkeit, Ruud Van Deursen, Lorenz C Blum, and Jean-Louis Reymond. Enumeration of 166 billion organic small molecules in the chemical universe database gdb-17. Journal of chemical information and modeling, 52(11):2864–2875, 2012.

[2] Raghunathan Ramakrishnan, Pavlo O Dral, Matthias Rupp, and O Anatole von Lilienfeld. Quantum chemistry structures and properties of 134 kilo molecules. Scientific Data, 1, 2014.

[3] Vignac, C., & Frossard, P. (2021). Top-N: Equivariant set and graph generation without exchangeability. arXiv preprint arXiv:2110.02096.


##Reviewer 2
Comment:
Certainly, LSGM cannot be directly applied to graph data. The key concern is the high similarity of the proposed approach to LSGM (The figure 1 of this paper and the figure 1 in LSGM paper show the same model framework). The key modification in the presented approach is the Gaussian prior in VGAE is replaced by a score network (proposed in LSGM). The missing evaluation of "novelty" in the arXiv paper [3] should not be an excuse of the low novelty presented in this paper. Molecular graph generation has been studied in a bunch of papers. It is necessary for new approaches to show good performance in terms of the popularly used evaluation metrics.

##Author
Thanks for the further feedback.
Q1. the high similarity of the proposed approach to LSGM.

Response: Our work is based on LSGM so the illustration of our model is similar to that of LSGM. We have updated our illustration. Please feel free to check our updated paper and see if it alleviates your concern. As we mentioned, it takes non-trivial work to design the prior, the encoder, and the decoder. They are all important for the model to work, though it may not be necessary to show all these designs in the illustration.

Q2. evaluation of "novelty".

Response: We want to emphasize that we are not looking for an "excuse" here. We hope you agree that most evaluation metrics have their weaknesses: namely, the best model may not achieve the best value according to some metric. Therefore, correct interpretations of performance values are critically important for the development of the field.

The purpose of training a generative model is to generate graphs that are from the same distribution as training graphs. As we have argued, novelty is not a good evaluation metric for QM9 when the training fraction is large: a high novelty value often means the learned distribution is too dispersed. Our model also shows good performance on novelty when the training fraction is small. Please let us know if you find issues in our analysis.


-------------------------------------------------------------------
##Reviewer 3
Summary:
This paper focuses on applying diffusion models to graph generation tasks. By utilizing the structure of VGAE and replacing its Gaussian prior to an attention-based SGM, the proposed method can generate novel graphs without fixing the node permutation. Extensive experiments are conducted to demonstrate the overall superior performance in generating novel graphs.

Strengths And Weaknesses:
Strengths: 
1) The method leverages diffusion method coupled with variational graph autoencoder, which is a novel and effective attempt in the graph generation area. 
2) The proposed methods replace the over-simple prior by score-based diffusion model that can attain both expressiveness and flexibility. 
3) Extensive experiments are conducted to validate the generation quality of the proposed method against others. Weaknesses: 
1) The manuscript does not address what are advantages of adopting diffusion methods in graph generation, which makes the work more like an incremental work. 
2) The evaluation metrics is a little outdated, the authors could consider adopting more advanced graph generation metrics. 
3) The authors claim that “By diffusing only the node vectors, NVDiff can learn to generate larger graphs with high quality in one-shot”, however, the experiment only involves generating relatively small graphs. 
4) The authors claim that the proposed methods enjoys faster sampling speed, but authors do not provide theoretical analysis and the experiment of model runtime only compares the proposed model with one method.

Questions:
1. Considering the scalability problem of the attention-based method, how does the proposed method perform on generating large graphs? The used graphs are relatively small (less than 500 nodes). In addition, could the authors also
2. In terms of the graph generation quality, the authors utilize standard MMD distances comparison in multiple static graph property distributions. However, these evaluations are a little outdated and it would be better to analyze the generation quality under the STOA graph evaluation metrics like proposed in [1].
3. It is a bit unclear why we should adopt diffusion model in deep graph generation. From the prospective of using a more meaningful prior, multiple papers [2, 3] in the past years have been proposed to replace the over-simple Gaussian prior in VAE, why should we adopt diffusion model instead?
4. Could author provide justifications on how the proposed method can boost the sampling speed? Based on my understanding, the graph generation is just based on the VGAE framework that samples a random variable from a latent distribution and applies dot product of the random variables.
[1] ON EVALUATION METRICS FOR GRAPH GENERATIVE MODELS, ICLR 2022 [2] Diagnosing and Enhancing VAE Models, ICLR 2019 [3] Learning Hierarchical Priors in VAEs, NeurIPS 2019

Limitations:
I do not see any potential negative societal impact of the work.

Ethics Flag: No
Soundness: 3 good
Presentation: 3 good
Contribution: 3 good
Rating: 6: Weak Accept: Technically solid, moderate-to-high impact paper, with no major concerns with respect to evaluation, resources, reproducibility, ethical considerations.
Confidence: 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.
Code Of Conduct: Yes


##Author
Thank you for your feedback! We sincerely appreciate your feedback and would like to answer your questions below.

Q1. the experiment only involves generating relatively small graphs, ..., how does the proposed method perform on generating large graphs?

Response: Compared with the one-shot baseline methods, our model is already able to generate much larger graphs. For example, EDP-GNN and GDSS only experiment on datasets with nodes less than 40. Our work considers Community and Ego datasets that contain graphs with at most 399 nodes. Our model in general outperforms all the one-shot generative baselines in generation tasks with large graphs.

As a separate point, diffusion-based graph generative models are often focused on small graphs (e.g. molecule graphs). Our method has expanded the applicable scope of these models in terms of graph sizes.

Q2. it would be better to analyze the generation quality under the STOA graph evaluation metrics

Response: We follow the source code provided by [1] to calculate the new evaluation metrics. The results in the table below still indicate the advantage of the proposed model: it performs the best on three out of four datasets and has significant improvements on two datasets. Only on the fourth dataset, its performance is slightly worse than EDP-GNN but better than all other models.

            Com-small	      Com	            Ego-small	Ego
GraphRNN	0.997 +- 0.010	1.452 +- 0.092	1.094 +- 0.003	0.192 +- 0.002
GRAN	0.701 +- 0.093	1.406 +- 0.191	1.095 +- 0.003	0.196 +- 0.008
GraphCNF	0.876 +- 0.138	1.356 +- 0.261	1.094 +- 0.002	OOM
EDP-GNN	0.798 +- 0.159	1.416 +- 0.133	1.095 +- 0.002	0.189 +- 0.001
GDSS	0.858 +- 0.166	1.203 +- 0.353	1.097 +- 0.001	0.295 +- 0.069
NVDiff	0.688 +- 0.144	0.982 +- 0.155	1.092 +- 0.002	0.195 +- 0.004
Q3. why should we adopt diffusion model instead?

Response: Previous study [4] has shown that the prior of a hierarchical VAE still cannot match the flexibility of diffusion priors, so it is a promising direction to apply diffusion models to graph generation tasks.

In graph generation tasks, diffusion-based models also have advantages over previous one-shot graph generation methods such as VGAE and normalizing flows: diffusion models have more freedom in architecture design and can learn much more flexible representations.

However, diffusion methods (e.g. EDP-GNN, GDSS) suffer from slow sampling speed in graph tasks and have difficulties in generating relatively large graphs. We address these issues by learning diffusion-based latent vectors for nodes only. In particular, we innovate the architecture design (Section 3.3) to model node vectors. Our method can learn much more flexible node vectors than VGAE. It needs much less computation than EDP-GNN and GDSS. Our model achieves premium model performances in a series of graph generation tasks.

Q4. how the proposed method can boost the sampling speed.

Response: The diffusion process dominates the computation time and is often slow due to multiple denoising steps. The time complexity of the diffusion process is , where  is the number of function calls to the noise conditional score network and N is the number of nodes in a graph. In our ODE-based sampling,  in most cases. According to our analysis, competing methods (EDP-GNN and GDSS) have similar time complexities (we don't see their analysis in their work).

Our speed gain mainly comes from reducing the number of diffusion steps . Because we model graphs in a smaller latent space, which makes the generation task easier, we can greatly reduce the number of diffusion steps (e.g. from 1000 to 70). This argument is also supported by the LSGM paper.

We have updated the results on runtime to using the EGO dataset because its graphs have larger sizes than the previous dataset, and the comparison is more meaningful. We also include comparisons against the GDSS model. Note that the source code of GDSS became publicly available after the paper submission deadline. We find our method is much faster than both GDSS and EDP-GNN.

References:

[1] Thompson, R., Knyazev, B., Ghalebi, E., Kim, J., & Taylor, G. W. (2021). On Evaluation Metrics for Graph Generative Models. In International Conference on Learning Representations.

[2] Dai, B., & Wipf, D. (2018). Diagnosing and Enhancing VAE Models. In International Conference on Learning Representations.

[3] Klushyn, A., Chen, N., Kurle, R., Cseke, B., & van der Smagt, P. (2019). Learning hierarchical priors in vaes. Advances in neural information processing systems, 32.

[4] Sinha, A., Song, J., Meng, C., & Ermon, S. (2021). D2c: Diffusion-decoding models for few-shot conditional generation. Advances in Neural Information Processing Systems, 34, 12533-12548.


